How to Delete Without a Trace: Certified Deniability in a Quantum World

Is it possible to comprehensively destroy a piece of quantum information, so that nothing is left behind except the memory of whether one had it at one point? For example, various works, most recently Morimae, Poremba, and Yamakawa (TQC 2024), show how to construct a signature scheme with certified deletion where a user who deletes a signature on m cannot later produce a signature for m. However, in all of the existing schemes, even after deletion the user is still able keep irrefutable evidence that m was signed, and thus they do not fully capture the spirit of deletion. In this work, we initiate the study of certified deniability in order to obtain a more comprehensive notion of deletion. Certified deniability uses a simulation-based security definition, ensuring that any information the user has kept after deletion could have been learned without being given the deleteable object to begin with; meaning that deletion leaves no trace behind! We define and construct two non-interactive primitives that satisfy certified deniability in the quantum random oracle model: signatures and non-interactive zero-knowledge arguments (NIZKs). As a consequence, for example, it is not possible to delete a signature/NIZK and later provide convincing evidence that it used to exist. Notably, our results utilize uniquely quantum phenomena to bypass the celebrated result of Pass (CRYPTO, 2003) showing that deniable NIZKs are impossible even in the random oracle model.

==> 03-techlemmas.tex <==
\section{Technical Results} \anote{Open to better names} \justin{I would only put things in here that seem independently useful and that are technically nontrivial. For example, the generalized z-twirl could just go in the preliminaries. Don't worry about it too much for now, though. We can think of better names/if we want to restructure to highlight anything once we have all the technical pieces written down.}

\begin{theorem}[Adaptive Classical Deletion]\label{thm:adpcladel}
   Consider the following experiment between a challenger and an adversary $\adve$.
   \paragraph{\underline{$\adpdel{\adve}{\lambda}$}}
   \begin{enumerate}
       \item For $i \in [\lambda]$, sample $x_i^0, x_i^1 \samp \zo^\lambda$ and $c_i \samp \zo$.
       \item Prepare the state \begin{equation*}
           \ket{\phi} \propto \bigotimes_{i \in [\lambda]} \left(\ket{x_i^0} + (-1)^{c_i}\ket{x_i^1}\right)
       \end{equation*}
       \item Submit $\ket{\phi}$ to $\adve$.
       \item The adversary $\adve$ outputs functions\footnote{The adversary can output the truth tables of the functions.} $f_i: \zo^\lambda \to \zo^{\ell_i(\lambda)}$, and strings $y_i \in \zo^{\lambda}, d_i^1 \in \zo^\lambda, d_i^2 \in \zo^{\ell_i(\lambda)}$ for $i \in [\lambda]$.
       \item For $i \in [\lambda]$, the challenger checks if $y_i \in \{x_i^0, x_i^1\}$ and if $c_i = d^1_i\cdot (x_i^0 \oplus x_i^1) \oplus d^2_i\cdot (f(x_i^0) \oplus f(x_i^1))$. If all the checks pass, the challenger outputs $1$. Otherwise, the challenger outputs $0$.
   \end{enumerate}

   Then, for any \emph{unbounded} adversary $\adve$, we have 
   \begin{equation*}
       \Pr[\adpdel{\adve}{\lambda} = 1] \leq \negl(\lambda).
   \end{equation*}
\end{theorem}

We give the following corollary, which can be considered a purified version of the above game, which streamlines some of our proofs.
\begin{corollary}\label{cor:adpcladel}
       Consider the following experiment between a challenger and an adversary $\adve$.
   \paragraph{\underline{$\adpdelpur{\adve}{\lambda}$}}
   \begin{enumerate}
\item The challenger initializes the registers $\mathsf{XV} = (\mathsf{XV}_i)_{i \in [\lambda]}$, $\mathsf{CV} = (\mathsf{CV}_i)_{i \in [\lambda]}$, $\mathsf{X} = (\mathsf{X}_i)_{i \in [\lambda]}$.
\item The challenger prepares the state 
\begin{equation*}
    \ket{\psi} \propto \sum_{\substack{(x_i^0, x_i^1)_{i \in [\lambda]},\\(c_i)_{i \in [\lambda]}}}  \ket{x_1^0}^{\mathsf{XV}_{1,0}} \ket{x_1^1}^{\mathsf{XV}_{1,1}} \cdots \ket{x_\lambda^0}^{\mathsf{XV}_{\lambda,0}} \ket{x_\lambda^1}^{\mathsf{XV}_{\lambda,1}}\otimes \ket{c_1}^{\mathsf{CV}_{1}} \cdots \ket{c_\lambda}^{\mathsf{CV}_{\lambda}} \otimes \left(\bigotimes_{i \in [\lambda]} \left(\ket{x_i^0} + (-1)^{c_i}\ket{x_i^1}\right)^{\mathsf{X}_i}\right)
\end{equation*}
over the registers $\mathsf{XV}, \mathsf{CV}, \mathsf{X}$.
       \item The challenger submits the register $\mathsf{X}$ to the adversary.

       \item The challenger measures the registers $\mathsf{XV}, \mathsf{CV}$ to obtain values $(x_i^0, x_i^1)_{i \in [\lambda]}, (c_i)_{i \in [\lambda]}$
       \item The adversary $\adve$ outputs functions $f_i: \zo^\lambda \to \zo^{\ell_i(\lambda)}$, and strings $y_i \in \zo^{\lambda}, d_i^1 \in \zo^\lambda, d_i^2 \in \zo^{\ell_i(\lambda)}$ for $i \in [\lambda]$.
       \item For $i \in [\lambda]$, the challenger checks if $y_i \in \{x_i^0, x_i^1\}$ and if $c_i = d^1_i\cdot (x_i^0 \oplus x_i^1) \oplus d^2_i\cdot (f(x_i^0) \oplus f(x_i^1))$. If all the checks pass, the challenger outputs $1$. Otherwise, the challenger outputs $0$.
   \end{enumerate}

   Then, for any \emph{unbounded} adversary $\adve$, we have 
   \begin{equation*}
       \Pr[\adpdel{\adve}{\lambda} = 1] \leq \negl(\lambda).
   \end{equation*}
\end{corollary}
\begin{proof}
    The game $\adpdelpurpl$ is simply a purification of $\adpdelpl$. Thus, the result follows by \cref{thm:adpcladel}.
\end{proof}

We now present the following result about compressed oracles. Informally, it says that on-the-fly simulation of the reprogrammed oracle $H'$, where $H'$ is the reprogramming of $H$ obtained by switching $H(a)$ and $H(b)$, is equivalent to simply switching these values once in the compressed oracle database.
\begin{theorem}[Switching In-Database is Equivalent to Reprogramming]\label{thm:switchunitary}
    Let $(\adve_1, \adve_2)$ be a two-stage (unbounded) oracle algorithm with $1$-bit output. Let $U_{\adve_1}, U_{\adve_2}$ be the unitaries of $\adve_1, \adve_2$, that act on the registers $\mathsf{A, B, X, Y, W, Z}$. $\mathsf{X,Y}$ denotes the query input-output registers, $\mathsf{W}$ denotes the internal state register and $\mathsf{Z}$ denotes the single bit final output register. Finally, $\mathsf{A,B}$ will contain the choice of switching/reprogramming points $a, b$.

    Let $U_{\adve_1}^{\mathsf{step}}, U_{\adve_2}^{\mathsf{step}}$ denote a single step of the adversaries. That is, we have 
    \begin{equation*}
        U_{\adve_i} = (\mathsf{CPhO} \circ U_{\adve_1}^{\mathsf{step}})^{\otimes k}
    \end{equation*}
    
    Then, define the database reprogramming unitaries 
    \begin{align*}
        &U_{\mathsf{dbswitch,int}}: \ket{a}_\mathsf{A}\ket{b}_\mathsf{B}\ket{D \cup (a, v_1) \cup (b, v_2)}_\mathsf{D} \mapsto \ket{a}_\mathsf{A}\ket{b}_\mathsf{B}\ket{D \cup (a, v_2) \cup (b, v_1)}_\mathsf{D} \\
         &U_{\mathsf{dbswitch}}^{\mathsf{A,B,D}} = \mathsf{StdDecomp}^{A,D} \circ \mathsf{StdDecomp}^{B,D}\circ U_{\mathsf{dbswitch,int}}^{\mathsf{A,B,D}}\circ\mathsf{StdDecomp}^{A,D} \circ \mathsf{StdDecomp}^{B,D} \circ \mathsf{Increase}^{\otimes 2}
    \end{align*}
    Also define the query reprogramming unitary.
    \begin{equation*}
        U_{\mathsf{qswitch}}^{A,B,X}: \ket{a}_{\mathsf{A}}\ket{b}_{\mathsf{B}}\ket{x}_\mathsf{X} \mapsto \begin{cases}
            \ket{a}_{\mathsf{A}}\ket{b}_{\mathsf{B}}\ket{b}_\mathsf{X}, \text{ if } x = a,\\
    \ket{a}_{\mathsf{A}}\ket{b}_{\mathsf{B}}\ket{a}_\mathsf{X}, \text{ if } x = b,\\
    \ket{a}_{\mathsf{A}}\ket{b}_{\mathsf{B}}\ket{x}_\mathsf{X}, \text{ otherwise}
        \end{cases}
    \end{equation*}

    Denote the final state of the registers in the on-the-fly reprogramming and in-database reprogramming experiments as follows.
    \begin{align*}
        &\ket{\psi} = \left(U_{\mathsf{qswitch}} \circ \mathsf{CPhO} \circ U_{\mathsf{qswitch}}\circ U_{\adve_2}^{\mathsf{step}}\right)^{\otimes k} \circ U_{\adve_1} \ket{\Vec{0}}\\
        &\ket{\psi'} = \left(\mathsf{CPhO} \circ U_{\adve_2}^{\mathsf{step}}\right)^{\otimes k} \circ U_\mathsf{dbswitch} \circ U_{\adve_1} \ket{\Vec{0}}.
    \end{align*}

    Then, we have
    \begin{equation*}
        \norm{(\ket{1}^\mathsf{Z}\bra{1}^\mathsf{Z}\otimes I) \ket{\psi}}^2 = \norm{(\ket{1}^\mathsf{Z}\bra{1}^\mathsf{Z}\otimes I) \ket{\psi'}}^2.
    \end{equation*}
    That is, the two experiments are perfectly indistinguishable.
\end{theorem}

\begin{lemma}\label{lem:general-ztwirl}
    Let $A\subset \{0,1\}^n$ be a subset and let $\ket{A_{0,s}^{\psi}} \coloneqq 1/\sqrt{|A|}\sum_{a\in A} (-1)^{a\cdot s}\ket{a} \otimes \ket{\psi_a} $. Then
    \[
        \sum_{s\in \{0,1\}^n} \ketbra{A_{0,s}^{\psi}} = \frac{1}{|A|} \sum_{a\in A} \ketbra{a} \otimes \ketbra{\psi_a} 
    \]
\end{lemma}
\begin{proof}
    We compute
    \begin{align*}
        \sum_{s\in \{0,1\}^n} \ketbra{A_{0,s}} 
        &=  \frac{1}{|A|}\sum_{s\in \{0,1\}^n} \sum_{a_1, a_2 \in A} (-1)^{(a_1 - a_2)\cdot s} \ket{a_1}\bra{a_2}\otimes \ket{\psi_{a_1}}\bra{\psi_{a_2}}
        \\
        &= \frac{1}{|A|}\sum_{a_1, a_2 \in A} \ket{a_1}\bra{a_2}\otimes \ket{\psi_{a_1}}\bra{\psi_{a_2}} \sum_{s\in \{0,1\}^n} (-1)^{(a_1 - a_2)\cdot s} 
        \\
        &= \frac{1}{|A|} \sum_{a \in A} \ket{a}\bra{a}\otimes \ketbra{\psi_a}
    \end{align*}
\end{proof}

==> 04-signatures-game.tex <==

\section{Signatures with Game-Based Certified Deniability}
In this section, we introduce a game-based security notion for signatures with certified deniability. Here, we consider an adversary who receives multiple signatures from a signing authority, and later deletes some of them. We require that once the adversary successfully deletes a signature for message $m$, it will not be able to convince \emph{any} sound verifier $\verfr$ that $m$ was signed. We re-emphasize that, crucially, we are considering security against any verifier $\verfr$, and not only the honest verification procedure of the signature scheme. In particular, the verifier and the adversary can share a quantum auxiliary input, and they can use any input/output format or protocol between them (for example, see \cref{sec:plainmodimp} for the plain model impossibility result where $\adve$ and $\verfr$ use a separate, special purpose signature scheme between them).

Now we formally give our security definition. Consider the following game between a challenger, an adversary $\adve$ and a (adversarial) verifier $\verfr$ (together with an auxiliary input setup algorithm $\mathsf{AuxSetup}$).

\paragraph{\underline{$\sigcdgame{\adve}{\verfr}{\lambda}$}}
\begin{enumerate}
    \item The challenger initializes a list $M = []$.
    \item The challenger samples $(\sk, \verkey) \samp \Gen(1^\lambda)$.
    \item The challenger initializes $(\regi{aux, adv}, \regi{aux, ver}) \samp \mathsf{AuxSetup}(vk), \verkey$ and submits $\regi{aux,adv},\verkey$ to the adversary $\adve$.
    \item For polynomially many rounds, the adversary queries for signatures by outputting a message $m$. For each query, the challenger samples $\regi{sig} \samp \Sign(\sk, m)$ and submits $\regi{sig}$ to the adversary. It also adds $m$ to the list $M$.
    \item The adversary outputs two count values $k_1, k_2$ with $k_1 + k_2 = |M|$, and two registers, $(m_i^\mathsf{del}, \regi{cert, i})_{i \in [k_1]}$ and $(m_i^\mathsf{forged}, \regi{forged, i})_{i \in [k_2]}$.
    \item The challenger executes $\DelVer(\sk, m^\mathsf{del}_i, \regi{cert, i})$ for $i \in [k_1]$. For each test, if the output is $1$, $m_i$ is removed from $M$; if the output is $0$, the challenger outputs $0$ and terminates.
    \item The challenger executes $\verfr(\verkey, \regi{aux,ver}, m_i^\mathsf{forged}, \regi{forged, i})$ for $i \in [k_2]$. If any of them outputs $0$, the challenger outputs $0$ and terminates.

    \item The challenger checks if $m_i^\mathsf{forged} \in M$ for all $i \in [k_2]$. If true for all, the challenger outputs $0$. Otherwise, the challenger outputs $1$.
\end{enumerate}

\begin{definition}[Game-Based Certified Deniability for Signatures]\label{def:cden-sigs-game}
    A revocable signature scheme $(\Gen,\allowbreak \Sign,\allowbreak \Verify,\allowbreak \Del,\allowbreak \DelVer)$ is \emph{game-based certifiably deniable} if 
    for any QPT adversary $\adve$ and any QPT \emph{sound} verifier $\verfr$ (with setup $\mathsf{AuxSetup}$), we have
    \begin{equation*}
        \Pr[\sigcdgame{\adve}{\verfr}{\lambda} = 1] \leq \negl(\lambda).
    \end{equation*}
\end{definition}
In the QROM model, we give the adversary $\adve$, the setup $\mathsf{AuxSetup}$ and the verifier $\verfr$ access to the random oracle.

Finally, we formalize the notion of a \emph{sound verifier} used in our definitions. \begin{definition}\label{def:sound-sig-ver}
Let $(\Gen,\allowbreak \Sign)$ be a signature scheme.
For a verification algorithm $\verfr$ (along with an auxiliary setup algorithm $\mathsf{AuxSetup}$), consider the following game between a challenger and an adversary $\adve$.

\paragraph{\underline{$\soundvergame{\adve}{\verfr}(1^\lambda)$}}
\begin{enumerate}
\item The challenger samples $\regi{aux,adv}, \regi{aux,ver} \samp \mathsf{AuxSetup}(1^\lambda)$.
    \item The challenger samples $\sk, \verkey \samp \Gen(1^\lambda).$
    \item The challenger samples $\sig \samp \Sign(\sk, \mdum)$ and submits $\verkey, \regi{aux,adv}, \sig$ to $\adve$.
    \item The adversary $\adve$ outputs a message $m \neq \mdum$ and a quantum register $\regi{}$.
    \item The challenger runs $\verfr$ on $\verkey, \regi{aux,ver},m, \regi{}$ and outputs its decision bit.
\end{enumerate}

We say that the verifier $\verfr$ (with $\mathsf{AuxSetup}$) is \emph{sound} if for any QPT adversary $\adve$, we have 
\[
\Pr[\soundvergame{\adve}{\verfr}(1^\lambda) = 1] \leq \negl(\lambda)
\]
\end{definition}

Note that according to our definition, the verifier needs to be sound only against adversaries that receive a single signature for a fixed message $\mdum$. This is a strictly weaker requirement than, e.g., requiring that $\verfr$ satisfy existential unforgeability. Thus, the corresponding security definition becomes stronger by protecting against a larger set of adversarial verifiers.
% Thus, our certified deletion security notions apply for a very large set of verifiers. Observe that stricter requirements for $\verfr$ would shrink the set of verifiers against which our certified deletion security notion would apply, thus making the security guarantees weaker.

We also define a weaker version of our game-based certified deletion  notion called \emph{one-time game-based certified deniability}, with the associated security game denoted $\sigcdotgame{\adve}{\verfr}{\lambda}$. In this setting, the adversary can query for a single signature, which it has to delete at the end (that is, $k_1 = 1$ and $k_2 = 0$). Further, we allow the signature scheme to output a deletion verification key along with the signature\footnote{That is, this key is on per-signature basis}, but the deletion verification key is sent directly to the challenger and not the adversary since we are in the private deletion verification setting. We will first give a construction that satisfies the one-time security, and later we show how to upgrade to full security generically.
\subsection{One-Time Construction with Classical Certificates}
In this section, we give our certified deniable signature scheme with classical certificates of deletion.
\begin{construction}[$\sigcdot$]\label{constr:sig-cden}
   Let $\digsig$ be a EUF-CMA secure signature scheme with deterministic signatures. Let $H: \zo^{\lambda + m(\lambda) + \log(\lambda)} \to \zo^{2\cdot m(\lambda) + 2\lambda + 2\log(\lambda)}$ denote a random oracle where $m(\lambda)$ is the message length. The construction is as follows.
    \begin{itemize}
            \item \underline{$\Gen(1^\lambda)$:}
            \begin{enumerate}
                \item Sample $\sk, \verkey \samp \digsig.\Gen(1^\lambda).$
                \item Output $\sk, \verkey$.
            \end{enumerate}
        \item \underline{$\Sign(\sk, m)$:}
        \begin{enumerate}
        \item Sample $x_i^0, x_i^1 \samp \zo^\lambda$ and $c_i \samp \zo$ for $i \in [\lambda]$.
        \item Secret share the message $m$ as $m_1, \dots, m_\lambda \samp \addsh{\lambda}{m}$.
        \item For $i \in [\lambda]$, prepare the state $\propto \ket{x^0_i} + (-1)^{c_i}\ket{x^1_i}$ in register $\mathsf{X}_i$. Define $\mathsf{X} = (\mathsf{X}_i)_{i \in [\lambda]}$.
        \item Initialize the registers $\mathsf{S} = (\mathsf{S}_i)_{i \in [\lambda]}$ to $\ket{\zvec}$.
        \item  For $i \in [\lambda]$, apply the mapping\footnote{We encode the values $i \in [\lambda]$ as $\log(\lambda)$-bit strings when used as part of input to $H$.}
        \begin{equation*}
            \ket{x}_{\mathsf{X}_i} \otimes \ket{\zvec}_{\mathsf{S}_i} \mapsto \ket{x}_{\mathsf{X}_i} \otimes \ket{\dss.\Sign(\sk, H(x || m_i || i))}_{\mathsf{S}_i}
        \end{equation*}
        to the registers $(\mathsf{X}_i, \mathsf{S}_i)$. This results in the state
        \begin{equation*}
           \propto \bigotimes_{i \in [\lambda]} \left(\ket{x_0^i}_{\mathsf{X}_i}\ket{\dss.\Sign(\sk, H(x^0_i || m_i || i))}_{\mathsf{S}_i}  + \ket{x_1^i}_{\mathsf{X}_i}\ket{\dss.\Sign(\sk, H(x^1_i || m_i || i))}_{\mathsf{S}_i}  \right)
        \end{equation*}
        \item For $i \in [\lambda]$, compute $a^1_i = (x_i^0 \oplus x_i^1)$ and $a^2_i = (\dss.\Sign(\sk,\allowbreak H(x^0_i || m_i || i)) \oplus \dss.\Sign(\sk,\allowbreak H(x^1_i || m_i || i)))$.
            \item If $m \neq \mdum$, output $(\mathsf{X}, \mathsf{S}, (m_i)_{i \in [\lambda]})$ as the signature and $\delkey = (a^1_i, a^2_i, c_i)_{i \in [\lambda]}$ as the deletion key. Otherwise (if $m = \mdum$), output $(\mathsf{X}, \mathsf{X}, (m_i)_{i \in [\lambda]}, (x_i^0, x_i^1)_{i \in [\lambda]},\allowbreak (a^1_i, a^2_i, c_i)_{i \in [\lambda]})$ as the signature.
        \end{enumerate}
        
        \item \underline{$\Verify(\verkey, m, \regi{sig})$:} 
        \begin{enumerate}
            \item Parse $((\regi{X,i})_{i \in [\lambda]}, (\regi{S,i})_{i \in \lambda}, (m_i)_{i \in [\lambda]}) = \regi{sig}$.
            \item Check if $\bigoplus_{i \in \lambda} m_i = m$. Output $0$ and terminate if not.
            \item For $i \in [\lambda]$, coherently evaluate $\dss.\Verify(\verkey, \cdot || m_i || i, \cdot)$ on the registers $(\regi{X,i}, \regi{S,i})$, then measure the outcome. If the measurement outcome is $1$ for all $i \in [\lambda]$, output $1$. Otherwise, output $0$.
        \end{enumerate}
        
        \item \underline{$\Del(\regi{sig})$:} 
        \begin{enumerate}
        \item Parse $((\regi{X,i})_{i \in [\lambda]}, (\regi{S,i})_{i \in \lambda}, (m_i)_{i \in [\lambda]}) = \regi{sig}$.
            \item For $i \in [\lambda]$, apply $\qft$ to $(\regi{X,i}, \regi{S,i})$ and measure these registers to obtain $d_i^{1}, d_{i}^2$.
            \item Output $(d_i^{1}, d_{i}^2)_{i \in [\lambda]}$.
        \end{enumerate}
        
        \item \underline{$\DelVer(\delkey, \cert)$:} 
        \begin{enumerate}
        \item Parse $(a^1_i, a^2_i, c_i) = \delkey$ and $(d_i^{1}, d_{i}^2)_{i \in [\lambda]} = \cert$.

        \item For $i \in [\lambda]$, verify if $d_i^1\cdot a^1_i \oplus d_i^2\cdot a^2_i = c_i$. Output $1$ if all the verifications pass. Otherwise, output $0$.
        \end{enumerate}
    \end{itemize}

\end{construction}

\begin{theorem}\label{thm:sig-cden-euf-sec}
    \cref{constr:sig-cden} satisfies existential unforgeability against chosen message attacks.
\end{theorem}

\begin{theorem}\label{thm:sig-cden-cd-sec}
    \cref{constr:sig-cden} satisfies one-time game-based certified deniability security.
\end{theorem}

\subsection{Proof of EUF-CMA Security}
In this section, we prove \cref{thm:sig-cden-euf-sec}. \anote{todo}
\subsection{Proof of One-Time Game-Based Certified Deniability}
In this section, we prove \cref{thm:sig-cden-cd-sec}. We will do our proof in the compressed oracle model (\cref{sec:prelim-compor}). Consequently, any reference to oracle algorithms (such as the adversary $\adve$, the verifier $\verfr$) will implicitly mean their compressed oracle versions.

Let $\verfr$ be a sound verifier (\cref{def:sound-sig-ver}) and $\adve$ be a query-bounded adversary. Suppose for a contradiction that $\adve$ wins the certified deletion game with non-negligible probability, that is, there exists a polynomial $p(\cdot)$ such that $\Pr[\sigcdotgame{\adve}{\verfr}{\lambda} = 1] \geq 1/p(\lambda)$ for infinitely many $\lambda > 0$.

First, we completely purify the experiment $\sigcdotgame{\adve}{\verfr}{\lambda}$ by converting any random sampling\footnote{This includes the ones made by the challenger, such as sampling the keys of the scheme} in the game into measurements, and delaying all the measurements. Accordingly, we also write $U_{\adve}$ and $U_{\verfr}$ to denote the unitary part of the purified versions of the adversary $\adve$ and the verifier $\verfr$. Let $\mathsf{P}_1^*$ denote the projection onto $\ketbra{1}{1}$ on the decision qubit register of $\verfr$\footnote{That is, $\verfr$ acts by applying $U_{\verfr}$ and applying the measurement $\{\mathsf{P}_1^*, I - \mathsf{P}_1^*\}$ on the first output qubit}.

Now, define the following registers
\begin{itemize}
    \item $\mathsf{XV}$, the $2\lambda\cdot\lambda$-qubit register containing the values $(x_i^0, x_i^1)_{i \in [\lambda]}$.
    \item $\mathsf{CV}$, the $2\lambda$-qubit register containing the values $(c_i)_{i \in [\lambda]}$,
    \item $\mathsf{M}$, the $m(\lambda)$-qubit register that contains the message chosen by the adversary
    \item $\mathsf{MS}$, the $\lambda\cdot m(\lambda)$-qubit register that contains the shares obtained by secret sharing $m$,
    \item $\mathsf{W}$, the deletion certificate output register,
    \item $\mathsf{Z}$, the forged signature output register\footnote{This will be fed to $\verfr$} of the adversary,
    \item $\mathsf{D}$, the compressed oracle database register,
    \item $\regi{}$, the remaining register containing all the other registers not named above (e.g. rest of the purification registers, auxiliary registers of $\adve$ and $\verfr$ and so on)
\end{itemize}

We note that the challenger can initialize the registers $\mathsf{XV}, \mathsf{CV}$ before the adversary is run. Thus, let $\ket{\chi}$ be the state of the above registers once the challenger performs the initialization, then we have
\begin{equation*}
    \ket{\chi} \propto  \left(\sum_{\substack{(x_i^0, x_i^1)_{i \in [\lambda]},\\(c_i)_{i \in [\lambda]}}}  \ket{x_1^0} \ket{x_1^1} \cdots \ket{x_\lambda^0} \ket{x_\lambda^1}\otimes \ket{c_1} \cdots \ket{c_\lambda}\right) \otimes \ket{\{\}}_{\mathsf{D}} \otimes \ket{\chi_{rest}}_{\mathsf{M},\mathsf{MS},\mathsf{W}, \mathsf{Z},\mathsf{R}}
\end{equation*}
where $\ket{\{\}}_{\mathsf{D}}$ denotes the empty initial state of the compressed oracle database.
Now, let $\ket{\psi}$ be the state of the registers above right after the adversary $\adve$ completely yields\footnote{That is, right before the deletion certificate verification and $\verfr$ is run.}. Write $\ket{\psi}$ as
\begin{equation*}
    \ket{\psi} = \sum_{\substack{(x_i^0, x_i^1)_{i \in [\lambda]}, \\ (c_i)_{i \in \lambda},\\ m, (m_i)_{i \in [\lambda]}, \\ w, z, D, p }} \beta_{\substack{(x_i^0, x_i^1)_{i \in [\lambda]}, \\ (c_i)_{i \in [\lambda]},\\ m, (m_i)_{i \in [\lambda]}, \\ w, z, D, p }} \ket{x_1^0} \ket{x_1^1} \cdots \ket{x_\lambda^0} \ket{x_\lambda^1}\otimes \ket{c_1} \cdots \ket{c_\lambda} \otimes \ket{m} \otimes \ket{m_1}\cdots \ket{m_\lambda} \otimes \ket{w} \otimes \ket{z} \otimes \ket{D} \otimes \ket{p}
\end{equation*}
Note that $\ket{\psi}$ will be obtained from $\ket{\chi}$ by first running $\mathsf{AuxSetup}$ and the first part (i.e. message selection) of the adversary, then running the signing phase of the challenger (which reads the prepared registers $\mathsf{XV},\mathsf{CV}$ for the relevant values) and finally running the second part of the adversary.

We will write $\Vec{x}$ to denote the tuple of variables $(x_i^0, x_i^1)_{i \in [\lambda]}$, and we similarly define $\Vec{m}, \Vec{c}$ and so on. We also define the following sets. We define $\mathsf{BADCERT}_{\Vec{x}, \Vec{m}, \Vec{c}, D, p}$ to be the set of certificates that are not valid, that is, $w = (w_1, w_2)$ that do not satisfy $c_i = w_1\cdot (x_i^0 \oplus x_i^1) \oplus w_2\cdot(\dss.\Sign(\sk, H(x^0_i || m_i)) \oplus \dss.\Sign(\sk, H(x^1_i || m_i)))$ for all $i \in [\lambda]$. We define $\mathsf{GOODCERT}_{\Vec{x}, \Vec{m}, \Vec{c}, D, p}$ to be the complement of $\mathsf{BADCERT}_{\Vec{x}, \Vec{m}, \Vec{c}, D, p}$. We also define the sets $\mathsf{MISS}_{i, \Vec{x}, \Vec{m}}$ for $i \in [\lambda]$ consisting of compressed oracle databases that does not contain any of the inputs $x_i^0 || m_i || i, x_i^1 || m_i || i, x_i^0 || (m_i \oplus m \oplus \mdum) || i, x_i^1 || (m_i \oplus m \oplus \mdum) || i$. If a database $D$ misses the above values for both $i = j_1$ and $i = j_2$ with $j_1 < j_2$, we put $D$ in $\mathsf{MISS}_{j_1, \Vec{x}, \Vec{m}}$. Finally, we define $\sigfulldb$ to be the set of compressed oracle databases that contains at least one of $x_i^0 || m_i || i, x_i^1 || m_i || i, x_i^0 || (m_i \oplus m \oplus \mdum) || i, x_i^1 || (m_i \oplus m \oplus \mdum) || i$ for all $i \in [\lambda]$.

Henceforth, we will not explicitly write the dependencies on variables such as $x_i^0, x_i^1$ and they will be implicit. Similarly, we will not explicitly write out the variables in summations unless they are restricted (e.g. over a subset of their domains) and also omit denoting the register names explicitly.

Now, we define the following subnormalized states.
\begin{align*}
    &\ket{\psi_{\mathsf{rej}}} = \sum_{w \in \mathsf{BADCERT}} \beta \ket{\Vec{x}} \ket{m} \ket{\Vec{m}} \ket{w} \ket{z} \ket{D} \ket{p} \\
    &\ket{\psi_{0}} = \sum_{\substack{w \in \mathsf{GOODCERT},\\ D \in \sigfulldb}} \beta \ket{\Vec{x}} \ket{m} \ket{\Vec{m}} \ket{w} \ket{z} \ket{D} \ket{p} \\
    &\ket{\psi_{i}} = \sum_{\substack{w \in \mathsf{GOODCERT},\\ D \in \mathsf{MISS}_i}} \beta \ket{\Vec{x}} \ket{m} \ket{\Vec{m}} \ket{w} \ket{z} \ket{D} \ket{p} \text{ for } i \in [\lambda]
\end{align*}

Observe that $\mathsf{BADCERT}, \mathsf{GOODCERT}$ partitions the set of certificate strings, and $\mathsf{MISS}_1, \dots, \mathsf{MISS}_\lambda$, $\sigfulldb$ partitions the set of compressed oracle databases. Thus, we have
\begin{equation*}
    \ket{\psi} = \ket{\psi_{\mathsf{rej}}} + \ket{\psi_0} + \ket{\psi_1} + \dots + \ket{\psi_\lambda}.
\end{equation*}

\begin{claim}\label{claim:sigclasdelpsii}
    $\ket{\psi_i} \perp \ket{\psi_j}$ for all $i \neq j \in \{0, 1, \dots, \lambda\}$.
\end{claim}
\begin{proof}
    Since the sets $\mathsf{MISS}_1, \dots, \mathsf{MISS}_\lambda$, $\sigfulldb$ constitute a partitioning of the set of all databases, $\ket{\psi_i}$ and $\ket{\psi_j}$ are states with disjoint supports, therefore the result follows.
\end{proof}

\begin{claim}\label{claim:sigclasdelpsirej}
    $\ket{\psi_\mathsf{rej}} \perp \ket{\psi_i}$ for all $i \in \{0, 1, \dots, \lambda\}$.
\end{claim}
\begin{proof}
    Since $\mathsf{BADCERT}$ and $\mathsf{GOODCERT}$ constitute a partitioning of the set of all certificate strings, $\ket{\psi_j}$ for any $i \in \{0, 1, \dots, \lambda\}$ and $\ket{\psi_\mathsf{rej}}$ are states with disjoint support, therefore the result follows.
\end{proof}

\begin{claim}\label{claim:sigclasdelpsi0}
    $\norm{\ket{\psi_0}} \leq \negl(\lambda)$.
\end{claim}
\begin{proof}
We will show that if $\ket{\psi_0}$ has non-negligible norm, we can break the information-theoretic deletion security game in \cref{thm:adpcladel} (more precisely, \cref{cor:adpcladel}).

Consider the following adversary $\adve'$.
\paragraph{\underline{$\adve'$}}
\begin{enumerate}
\item Receive the register $\mathsf{X}$ from the challenger.
\item Prepare the compressed oracle database register $\mathsf{D}$. Henceforth, instructions below with access to the quantum random oracle $H$ will be simulated using $\mathsf{D}$.
\item Sample $\sk, \verkey \samp \sigcdot.\Gen(1^\lambda)$.
\item $\regi{aux,adv}, \regi{aux,ver} \samp \mathsf{AuxSetup}^H(\verkey)$.
\item Simulate $\adve^H$ by submitting $\regi{aux,adv}, \verkey$ to it. It yields a message $m$.


\item Simulate $\regi{sig}, \delkey \samp \sigcdot.\Sign(\sk, m)$ but using $\mathsf{X}$ received from the challenger instead of $\sigcdot.\Sign$ preparing its own $\mathsf{X}$ register.
\justin{Why doesn't this record one $x$ value from each index (in superposition) to $D$?}
\anote{You mean receiving $X$ from deletion game and doing this? It does record one value from each index, true. So at this point you can extract one value for each index. But, to produce a good certificate, you must "forget" any preimage for at least one index.}
\justin{But the only way to "forget" an entry in the RO database is to query it again (thereby invoking the compression algorithm). Measuring the signature in the hadamard basis doesn't do this, so it can't "forget" the entry from the database. I would actually expect this to result in a bad certificate, since the signature is entangled with the database. Actually, if the database is in superposition, how do we check the certificate? The check seems to depend on $H$.}


\item Simulate $\adve^H$ by submitting $\regi{sig}$ to it. It yields a register $\regi{forged}$ and a certificate $\cert$.


\item\label{item:advepriforadpdel} Measure the compressed oracle register $\mathsf{D}$. Let $D$ be the outcome.

\item Choose a random subset of entries from $D$ of size $\lambda$, let $((z_i, v_i)_{i \in [\lambda]}$ denote the selected entries.

\item Set $D' = D$. Keep sampling uniformly random input-output pairs $(z, v)$ with $z \samp \zo^{\lambda + m(\lambda) + \log(\lambda)}, v \samp \zo^{2\lambda + 2\cdot m(\lambda) + 2\log(\lambda)}$ and adding them to $D'$ until $D'$ contains an entry for all possible inputs $\zo^{\lambda + m(\lambda) + \log(\lambda)}$.

\item For $i \in [\lambda]$, compute the function descriptions\footnote{As a truth table} for the functions $f_i$ defined as
\begin{equation*}
    f_i(z) = \digsig.\Sign(\sk, D'(z))
\end{equation*}

\item For each $i \in [\lambda]$, search the list $((z_i, v_i))_{i \in [\lambda]}.$ to find an element such that the last $\log(\lambda)$ bits of $z_i$ encodes the value $i$; if there is no such element, output $\perp$ and terminate.

\item Output $(z'_i)_{i \in [\lambda]}$ as the input values, $\cert$ as the certificates and $(f_i)_{i \in [\lambda]}$ as the functions.


\end{enumerate}

Let $\adve''$ be the version of $\adve'$ that is purified until \cref{item:advepriforadpdel}. Now consider the state of the registers of $\adve''$ and the challenger when $\adve''$ is playing $\adpdelpurpl$, right before $\adve''$ executes \cref{item:advepriforadpdel}. Observe that the state at this point is exactly the same as $\ket{\phi}$. Thus, when the adversary measures the compressed oracle register (and the certificate register, whose measurement had been delayed), with probability $\norm{\ket{\psi_0}}^2$, we get a compressed oracle database $D$ such that $D \in \sigfulldb$ and a certificate $w$ such that $w \in \mathsf{GOODCERT}$. Since $\adve$ is a QPT adversary, we have that $D$ has polynomially many entries, denote $q(\lambda)$. When $D \in \sigfulldb$, by definition, we know that for each $i \in [\lambda]$, there is at least one entry in $D$ where the input value starts with $x_i^0$ or $x_i^1$ and ends with $i$. Call such entries \emph{good}. Thus, when we randomly sample the subset $((z_i, v_i)_{i \in [\lambda]}$ of entries in $D$, with probability $\lambda/q(\lambda)$, it consists entirely of the good entries, one for each value of $i \in [\lambda]$. Thus, we can see that the adversary wins $\adpdelpurpl$ with probability at least 
\begin{equation*}
    \frac{\norm{\ket{\psi_0}}^2\cdot \lambda}{q(\lambda)}
\end{equation*}
Thus, by \cref{cor:adpcladel}, we get that $\norm{\ket{\psi_0}}^2$ must be negligible.
\end{proof}

Now we define $\ket{\phi}$, the state of the registers after applying $U_{\verfr}^\mathsf{Z, D, R}\otimes I$ to $\ket{\psi}$. Similarly, define $\ket{\phi_i} = (U_{\verfr}^\mathsf{Z, D, R} \otimes I)\ket{\psi_i}$ and $\ket{\phi_\mathsf{rej}} = (U_{\verfr}^\mathsf{Z, D, R} \otimes I)\ket{\psi_{\mathsf{rej}}}$. Also define $\mathsf{P}_{\mathsf{good-cert}}$ to be the projector on the register $\mathsf{W}$ onto $w$ such that $w \in \mathsf{GOODCERT}$. That is, $\mathsf{P}_{\mathsf{good-cert}} = \sum_{w \in \mathsf{GOODCERT}} \ket{w}^\mathsf{W}\bra{w}^\mathsf{W} \otimes I.$

\begin{claim}\label{claim:sigcladelnormphi}
    $\norm{(\mathsf{P}_1^*\otimes \mathsf{P}_{\mathsf{good-cert}}\otimes I) \ket{\phi}}^2 = \Pr[\sigcdotgame{\adve}{\verfr}{\lambda} = 1].$
\end{claim}
\begin{proof}
    
\end{proof}

We further define $\mathsf{P} = (\mathsf{P}_1^*\otimes \mathsf{P}_{\mathsf{good-cert}}\otimes I)$, $\ket{\phi'} = \mathsf{P}\ket{\phi}$, $\ket{\phi'_\mathsf{rej}} = \mathsf{P}\ket{\phi_\mathsf{rej}}$ and $\ket{\phi'_i} = \mathsf{P}\ket{\phi_i}$.

\begin{claim}
    $\ket{\phi'_i} \perp \ket{\phi'_j}$ for all $i \neq j \in \{0, 1, \dots, \lambda\}$.
\end{claim}

\begin{claim}\label{claim:sigcladelphipr0norm}
    $\norm{\ket{\phi'_0}} \leq \negl(\lambda)$.
\end{claim}
\begin{proof}
    
\end{proof}

\begin{claim}
    There exists $i^*_{\adve, \verfr} \in [\lambda]$ such that $\norm{\ket{\phi'_i}}^2 \geq \frac{1}{2\cdot \lambda \cdot p(\lambda)}$.
\end{claim}
\begin{proof}
First, it is easy to see that $\ket{\phi'_\mathsf{rej}} = 0$.
    Further, by the orthogonality results above, we get
    \begin{equation*}
        \norm{\ket{\phi'}}^2 = \norm{\ket{\phi'_0}}^2 + \norm{\ket{\phi'_1}}^2 + \dots + \norm{\ket{\phi'_\lambda}}^2.
    \end{equation*}

    By \cref{claim:sigcladelphipr0norm}, we have $\norm{\ket{\phi'_0}}^2 \leq 1/(2\cdot p(\lambda))$. By \cref{claim:sigcladelnormphi}, we have $\norm{\ket{\phi'}}^2 \geq 1/p(\lambda)$. Thus, by a simple averaging argument, the result follows.
\end{proof}

Now, for $i \in [\lambda]$, we define the in-database reprogramming unitaries $U_{i,0, \mathsf{dbswitch}}^{\mathsf{M}, \mathsf{XV}_{i,0}, \mathsf{MS}_i, \mathsf{D}}, U_{i,1, \mathsf{dbswitch}}^{\mathsf{M},\mathsf{XV}_{i,1}, \mathsf{MS}_i, \mathsf{D}}$ as in \cref{thm:switchunitary}, where the first unitary performs the reprogramming $x_i^0 || m_i || i \leftrightarrow x_i^0 || (m_i \oplus m \oplus \mdum) || i$ and the second one defines  $x_i^1 || m_i \leftrightarrow x_i^1 || (m_i \oplus m \oplus \mdum) || i$. We also define the short hand $U_{i, \mathsf{dbswitch}} = U_{i,0, \mathsf{dbswitch}}^{\mathsf{M}, \mathsf{XV}_{i,0}, \mathsf{MS}_i, \mathsf{D}} \circ U_{i,1, \mathsf{dbswitch}}^{\mathsf{M}, \mathsf{XV}_{i,0}, \mathsf{MS}_i, \mathsf{D}}$.

\begin{claim}
    For $i \in [\lambda]$, $U_{i, \mathsf{dbswitch}} \ket{\phi_i} = \ket{\phi_i}$.
\end{claim}
\begin{proof}
    
\end{proof}

We define $\mathsf{P}' = (\mathsf{P}_1^* \otimes I)\circ(U_\verfr \otimes I)\circ (U_{\textcolor{red}{i^*}, \mathsf{dbswitch}} \otimes I) \circ (\mathsf{P}_{\mathsf{good-cert}} \otimes I)$ and the following states.
\begin{align*}
    &\ket{\eta} =  \mathsf{P}'\ket{\eta}\\
    &\ket{\eta_i} =  \mathsf{P}'\ket{\eta_i} \text{ if } i \in [\lambda]\\
    &\ket{\eta_{\mathsf{rej}}} = \mathsf{P}'\ket{\eta_\mathsf{rej}}.
\end{align*}


\begin{claim}
    $\ket{\eta_i} \perp \ket{\eta_j}$ for all $i \neq j \in \{0, 1, \dots, \lambda\}$.
\end{claim}

\begin{claim}
    $\ket{\eta_\mathsf{rej}} \perp \ket{\eta_i}$ for all $i \in \{0, 1, \dots, \lambda\}$.
\end{claim}

\begin{claim}
    $\norm{\ket{\eta}}^2 \geq \frac{1}{2\cdot \lambda \cdot p(\lambda)}$.
\end{claim}
\begin{proof}
    
\end{proof}

Finally, we give an adversary $\adve'$ for the soundness game $\soundvergamepl$ (\cref{def:sound-sig-ver}) of the verifier $\verfr$. Let $H'$ denote the reprogrammed oracle defined as follows.
\begin{equation*}
    H'(z) = \begin{cases}
        &x_{i^*}^0 || (m_{i^*} \oplus m \oplus \mdum) || i^{*}, \text{ if } z = x_{i^*}^0 || m_{i^*} || i^{*},\\
        &x_{i^*}^0 || m_{i^*} || i^{*}, \text{ if } z = x_{i^*}^0 ||  (m_{i^*} \oplus m \oplus \mdum) || i^{*},\\
        &x_{i^*}^1 ||  (m_{i^*} \oplus m \oplus \mdum) || i^{*}, \text{ if } z = x_{i^*}^1 || m_{i^*} || i^{*},\\
        &x_{i^*}^1 || m_{i^*} || i^{*}, \text{ if } z = x_{i^*}^1 ||  (m_{i^*} \oplus m \oplus \mdum) || i^{*},
    \end{cases}
\end{equation*}

Then, we construct $\adve'$ as follows.

\paragraph{\underline{$\adve'$}}
\begin{enumerate}
    \item Receive $\regi{aux,adv}, \verkey$ from the challenger.
    \item Receive a signature for $\mdum$ from the challenger. Parse it as $(\regi{X}, \regi{S}, (m_i)_{i \in [\lambda]}, (x_i^0, x_i^1)_{i \in [\lambda]},\allowbreak (a^1_i, a^2_i, c_i)_{i \in [\lambda]})$.
    \item Simulate $\adve^{H}$ by submitting $\regi{aux,adv},\verkey$ to it. It yields a message $m$. 
    \item Simulate $\adve^{\textcolor{red}{H'}}$ by submitting $(\regi{X}, \regi{S}, (m_i)_{i \in [\lambda]}, (x_i^0, x_i^1)_{i \in [\lambda]})$. It yields a certificate $\cert$ and a register $\regi{forged}$.
    \item Parse $(d_i^{1}, d_{i}^2)_{i \in [\lambda]} = \cert$. For $i \in [\lambda]$, verify if $d_i^1\cdot a^1_i \oplus d_i^2\cdot a^2_i = c_i$. Output $m, \regi{forged}$ if all the verifications pass. Otherwise, output $\perp$.
\end{enumerate}

\begin{claim}\label{claim:advepribreaksver}
    $\Pr[\soundvergame{\adve'}{\verfr} = 1] \geq \frac{1}{2\cdot \lambda\cdot p(\lambda)}.$
\end{claim}

However, \cref{claim:advepribreaksver} is a contradiction to our assumption that $\verfr$ is a sound verifier. Thus, our initial hypothesis that $\adve$ wins the certified deletion game with non-negligible probability is incorrect. This completes the security proof.

\subsection{Generically Upgrading One-Time Security to Full Security}
In this section, we show how to construct a revocable signature scheme with game-based certified deniability (\cref{def:cden-sigs-game}) given a scheme that only satisfies one-time security.
\begin{construction}[$\sigcd$]\label{constr:sig-cden-mult}
Let $\sigcdot$ be a one-time revocable signature scheme, $\digsig$ be a EUF-CMA secure signature scheme, $\ske$ be a receiver-non-committing secret key encryption scheme and $\mac$ be a message authentication code. The construction is as follows.
    \begin{itemize}
        \item \underline{$\Gen(1^\lambda)$:}
    \begin{enumerate}
        \item Sample $\sk_g, \verkey_g \samp \digsig.\Gen(1^\lambda).$
        \item Sample $\sk_{enc} \samp \ske.\Gen(1^\lambda)$.
        \item Sample $\sk_{mac} \samp \mac.\Gen(1^\lambda)$.
        \item Output $(\sk_g, \sk_{mac}, \sk_{enc})$ as the signing key and $\verkey_g$ as the verification key.
    \end{enumerate}
        \item \underline{$\Sign(\sk, m)$:}
        \begin{enumerate}
       \item Parse $(\sk_g, \sk_{mac}, \sk_{enc}) = \sk$.
       \item Sample $\sk_{ot}, \verkey_{ot} \samp \sigcdot.\Gen(1^\lambda).$
       \item Sample $\sig_{vk} \samp \digsig.\Sign(\sk_{g}, \verkey_{ot})$.
       \item Sample $\regi{sig}, \delkey \samp \sigcdot.\Sign(\sk_{ot}, m)$.
       \item Sample $\ct \samp \ske.\enc(\sk_{enc}, \delkey)$.
       \item Sample $\tagg \samp \mac.\Sign(\sk_{mac}, \ct)$.
       \item Output $(\regi{sig}, \verkey_{ot}, \sig_{vk}, \ct, \tagg)$.
        \end{enumerate}
        
        \item \underline{$\Verify(\verkey, m, \regi{sig})$:} 
        \begin{enumerate}
            \item Parse $(\regi{sig}', \verkey_{ot}, \sig_{vk}, \ct, \tagg) = \regi{sig}$.
            \item Check if $\digsig.\Verify(\verkey, \verkey_{ot}, \sig_{vk})$ outputs $1$.
            \item Check if $\sigcdot.\Verify(\verkey, m, \regi{sig}')$ outputs $1$.
            \item Output $1$ if the checks pass. Otherwise, output $0$.
        \end{enumerate}
        
        \item \underline{$\Del(\regi{sig})$:} 
        \begin{enumerate}
        \item Parse $(\regi{sig}', \verkey_{ot}, \sig_{vk}, \ct, \tagg) = \regi{sig}$.
        \item $\regi{cert} \samp \sigcdot.\Del(\regi{sig}')$.
        \item Output $(\regi{cert}, \ct, \tagg)$.
        \end{enumerate}
        
        \item \underline{$\DelVer(\sk, \regi{cert})$:} 
        \begin{enumerate}
        \item Parse $(\sk_g, \sk_{mac}, \sk_{enc}) = \sk$.
        \item Parse $(\regi{cert}', \ct, \tagg) = \regi{cert}$.
        \item Check if $\mac.\Verify(\sk_{mac}, \ct, \tagg)$ outputs  $1$.
        \item $\delkey \samp \ske.\Dec(\sk_{enc}, \ct)$.
        \item Check if $\sigcdot.\DelVer(\delkey, \regi{cert})$ outputs $1$.
        \item Output $1$ if the checks pass. Otherwise, output $0$.
        \end{enumerate}
    \end{itemize}

\end{construction}

\anote{I think the same construction might give one-time simulation to full-simulation.}

\begin{theorem}\label{thm:genericupgradegame}
    Let $\sigcdot$ be a revocable signature scheme that satisfies one-time game-based certifiable deletion security. Then, $\sigcd$ is a revocable signature scheme that satisfies (full) game-based certifiable deletion security (\cref{def:cden-sigs-game}).
\end{theorem}

We note that by replacing $\ske$ with a receiver non-committing public-key encryption scheme and $\mac$ with a digital signature scheme, we can obtain a construction of revocable signature scheme with publicly-verifiable deletion from a one-time scheme with publicly-verifiable deletion. The proof follows similarly to our proof below.

\subsubsection{Proof of \cref{thm:genericupgradegame}}



==> 04-signatures.tex <==
\section{Signatures with Certified Deniability}\label{sec:sig-cden}

\justin{Our construction actually satisfies the NIZK notion, which should imply this (and be strictly stronger).}


Deniable authentication was initially defined by Dwork, Naor, and Sahai~\cite{STOC:DwoNaoSah98} using the simulation paradigm. Informally, a signature is deniable if it could be \emph{simulated} by using only public information. 

We follow a similar simulation-based paradigm which uses a real experiment $\sigcd_{\adv(\regi{\adv})}(\verkey)$. This experiment is parameterized by a QPT adversary $\adv$ who receives auxiliary input in register $\regi{\adv}$ and a key pair $(\sk, \verkey)$. It is defined as follows.
\begin{enumerate}
    % \item $\adv$ is initialized with register $\regi{\adv}$.
    % \item The challenger samples $(\sk, \verkey) \gets \Gen(1^\secpar)$ and sends $\verkey$ to $\adv$.
    % \item $\adv$ chooses a message $m$. The challenger samples $(\ket{\sigma}, \delkey) \gets \Sign(\sk,m)$ and sends $\ket{\sigma}$ to $\adv$.
    % \item $\adv$ outputs a certificate $\cert$ and a residual state $\rho$.
    % \item If $\DelVer(\delkey, \cert) = \Accept$, then output $\rho$. Otherwise, output $\bot$.
    \item $\adv$ is initialized with register $\regi{\adv}$ and $\verkey$. The challenger is initialized with 
    \item $\adv$ chooses a message $m^*$, which they send to the challenger. The challenger $(\ket{\sigma}, \delkey) \gets \Sign(\sk,m)$ and sends $\ket{\sigma}$ to $\adv$.
    \item $\adv$  gets access to a signing oracle for $\sk$, except it is not allowed to query on $m^*$. The signing oracle tracks the set of messages $M$ that it is queried on.
    \item $\adv$ outputs a certificate register $\regi{cert}$ and a register $\regi{\adv}$. %, potentially containing the residual signature state.
    \item If $\DelVer(\delkey, \regi{cert}) = \Accept$, then output $(M, \regi{\adv})$. Otherwise, output $(M, \bot)$.
\end{enumerate}
If working in an oracle model where the parties have access to an oracle $H$, then we denote the experiment as $\sigcd^H_{\adv(\regi{\adv})}$. 

\begin{definition}[Certified Deniability for Signatures: Plain Model]\label{def:cden-sigs}
    A revocable signature scheme $(\Gen,\allowbreak \Sign,\allowbreak \Verify,\allowbreak \Del,\allowbreak \DelVer)$ is \emph{certifiably deniable} if for every QPT adversary $\adv$, there exists a QPT simulator $\Sim$ such that for every QPT adversary $\adv$ with poly-size auxiliary input register $\regi{\adv}$,
    \begin{gather*}
       \left\{(\verkey, \sigcd_{\adv(\regi{\adv})}(\sk, \verkey)) : (\sk, \verkey) \gets \Gen(1^\secpar) \right\}
        \\
        \approx_c
        \\
        \left\{(\verkey, M_\Sim, \Sim^{\Sign(\sk, \cdot)}(\adv, \regi{\adv}, \verkey)) : (\sk, \verkey) \gets \Gen(1^\secpar) \right\}
    \end{gather*}
    where $M_\Sim$ is the set of messages on which $\Sim$ queries $\Sign(\sk, \cdot)$.
\end{definition}

The set $M$ acts as a way to restrict $\Sim$ from querying the signing oracle on $m^*$, which is only announced after $\adv$ sees $\verkey$. $\adv$ gets a free signing query on $m^*$ that is not recorded, but all of $\Sim$'s queries are recorded.

The above definition uses a \emph{selective} notion of security, where $\adv$ must declare which message it is going to delete before it sees other signatures.\footnote{Our definition actually is somewhat stronger than traditional selective notions, which would require the adversary to declare $m^*$ even before seeing $\verkey$.} A more general notion is \emph{adaptive} security, where $\adv$ is allowed to see many signatures before it decides which one to delete. Selective security can be upgraded to adaptive security using standard complexity leveraging techniques.


\paragraph{Certified Deniability in the QROM.} We may also define certified deniability in the CRS model or the QROM model. Following~\cite{C:Pass03}'s definition from the classical setting, a deniable simulator does \emph{not} have the ability to program the global random oracle; this is enforced by sampling a fresh random oracle before the experiment and including its description in the output of the experiment. Thus, any simulator which attempts to pretend that the oracle had different behavior is will be caught.

\begin{definition}[Certified Deniability for Signatures: QROM]\label{def:cden-sig-qrom}
    A revocable signature scheme $(\Gen,\allowbreak \Sign,\allowbreak \Verify,\allowbreak \Del,\allowbreak \DelVer)$ is \emph{certifiably deniable in the quantum random oracle model} if there exists a QPT simulator $\Sim$ such that for every QPT adversary $\adv$ with poly-size auxiliary input register $\regi{\adv}$,
    % \[
    %     \left\{\left( \sigcd^H_{\adv(\regi{\adv})}, O_H \right) : H\gets \mathsf{Func}(\cX, \cY) \right\}
    %     \approx_c
    %     \left\{\left(\Sim(\adv, \regi{\adv}, \verkey), O_H\right) : \begin{array}{c}
    %          H\gets \mathsf{Func}(\cX, \cY)  \\
    %         (\sk, \verkey) \gets \Gen^H(1^\secpar)
    %     \end{array} \right\}
    % \]
    \begin{gather*}
        \left\{(O_H, \verkey, \sigcd^H_{\adv(\regi{\adv})}(\sk, \verkey)) : \begin{array}{c}
             H\gets \mathsf{Func}(\cX, \cY)  \\
            (\sk, \verkey) \gets \Gen^H(1^\secpar)
        \end{array} \right\}
        \\
        \approx_c
        \\
        \left\{(O_H, \verkey, M_\Sim, \Sim^{H, \Sign^H(\sk, \cdot)}(\adv, \regi{\adv}, \verkey)) : \begin{array}{c}
             H\gets \mathsf{Func}(\cX, \cY)  \\
            (\sk, \verkey) \gets \Gen^H(1^\secpar)
        \end{array} \right\}
    \end{gather*}
    where $O_H$ denotes oracle access to $H$ and $M_\Sim$ is the set of messages on which $\Sim$ queries $\Sign^H(\sk, \cdot)$.
\end{definition}

We show in \cref{sec:fs-cden} how to obtain signatures with certified deniability by adding certified deniability to the Fiat-Shamir transformation.
\anote{Maybe move that construction and proof here? We can put all signature sections after all NIZK sections.
}

\justin{I was originally going to do all signatures together and all NIZKs together, but the signature construction is essentially the same as the NIZK construction and the proof is non-black-box in it.}

\anote{But currently sim-secure sig section will be just definitions. It's your call but IMO moving signature cons+proof there could be better (and since it will come after NIZK section, we can assume they know the NIZk construction and say that we asssume that). At the end actually we will probably move NIZK-based-signature proof to appendix due to page limit }

\justin{I was thinking about doing some reorganization anyway. The two options I was considering were (section:subsections):
\begin{itemize}
    \item \textbf{Simulation section:} signature definition, NIZK definition, FS construction, FS proof
    \\
    \textbf{Game-based section:} signature definition, NIZK definition, construction, proof
    % 
    \item \textbf{Simulation-based Definitions:} signatures, NIZKs
    \\
    \textbf{FS:} construction, proof
    \\
    \textbf{Game-based definitions}: signatures, NIZKs
    \\
    \textbf{classical certificates:} construction, proof
\end{itemize}
If we don't manage to fix the classical certificate construction in time, we can do (1) \textbf{definitions}: signatures, NIZKs and (2) \textbf{FS}: construction, proof.
\\
It's actually pretty reasonable to have a section just for definitions, especially considering definitions are one of our main contributions
}

==> 05-nizks.tex <==
\section{NIZKs with Certified Deniability}\label{sec:nizk-cden}


\justin{ZK seems separate from certified deniability because certified deniability only considers *after* the certificate is generated.}

\paragraph{Certified Deniability: Real Experiment.} Certified deniability follows the standard real/ideal paradigm of simulator-based definitions. The real experiment $\nizkcd_{\adv(\regi{\adv})}(s, w)$ is parameterized by an adversarial QPT algorithm with auxiliary input $\regi{\adv}$ and some NP statement and witness pair $(s, w)$.  $\nizkcd_{\adv(\regi{\adv})}(s, w)$ consists of the following distribution:
\begin{enumerate}
    \item Sample $(\delkey, \ket{\pi})\gets \Prove(s, w)$ and send $\ket{\pi}$ to the adversary.
    \item The adversary outputs two registers $(\regi{\cert}, \regi{\adv})\gets \adv(\regi{\adv}, \ket{\pi})$.
    \item If $\DelVer(\delkey, \regi{\cert})$ outputs accept, then the experiment outputs the adversary's residual state register $\regi{\adv}$. Otherwise, it outputs $\bot$.
\end{enumerate}
If working in an oracle model where the parties have access to an oracle $H$, then we denote the experiment as $\nizkcd^H_{\adv(\regi{\adv})}(s, w)$.


\begin{definition}[Certified Deniability for NIZKs: Plain Model]\label{def:nizk-cden-plain}
    A non-interactive argument system $(\Prove, \Verify, \DelVer)$ is \emph{certifiably deniable} if there exists a QPT simulator $\Sim$ such that for every QPT adversary $\adv$ with poly-size auxiliary input register $\regi{\adv}$ and every NP statement/witness pair $(s,w)$,
    \[
       \left \{\nizkcd_{\adv(\regi{\adv})}(s, w) \right\} 
       \approx_c 
       \left\{\Sim(s, \adv, \regi{\adv}) \right\}
    \]
\end{definition}

We may also define certified deniability in the CRS model or the QROM model. Following~\cite{C:Pass03}'s definition from the classical setting, a deniable simulator does \emph{not} have the ability to program the global random oracle; this is enforced by sampling a fresh random oracle before the experiment and including its description in the output of the experiment. Thus, any simulator which attempts to pretend that the oracle had different behavior is likely to be caught.

\begin{definition}[Certified Deniability for NIZKs: QROM]\label{def:nizk-cden-qrom}
    A non-interactive argument system $(\Prove, \Verify, \DelVer)$ is \emph{certifiably deniable in the quantum random oracle model} if there exists a QPT simulator $\Sim$ such that for every QPT adversary $\adv$ with quantum auxiliary input $\aux$ and every NP statement/witness pair $(s,w)$,
    \begin{gather*}
        \left\{ \left(\nizkcd^H_{\adv(\regi{\adv})}(s, w), O_H \right) : H\gets \mathsf{Func}(\cX, \cY) \right\} 
        \\
        \approx_c 
        \\
        \left\{\left(\Sim^H(s, \Adv, \regi{\adv}), O_H \right) : H\gets \mathsf{Func}(\cX, \cY) \right\}
    \end{gather*}
    where $O_H$ denotes oracle access to $H$.
\end{definition}


We show in \cref{sec:fs-cden} how to obtain NIZKs with certified deniability by adding certified deniability to the Fiat-Shamir transformation.

==> Notes/new.tex <==

\section{Definitions}
\begin{definition}[Signature Scheme with Deletion]
    A signature scheme with deletion consists of the following efficient algorithms.

    \begin{itemize}
        \item $\underline{\mathsf{Setup}(1^\lambda)}:$ Outputs a signing key $sk$ and a signature verification key $vk$.
        \item $\underline{\mathsf{Sign}(sk, m)}:$ On input the signing key $sk$ and a message $m$, outputs a classical signature for $m$.
                \item $\underline{\mathsf{Protect}(sk, sig)}:$ On input a classical signature $sig$, outputs a deleteable version of the signature.

        \item $\underline{\mathsf{SigVer}(vk, m, \regi{sig})}:$ On input the signature verification key, a message and a signature (either classical or deleteable), outputs $1$ or $0$.



        \item $\underline{\mathsf{DelVer}(dk, \regi{sig})}:$ On input the deletion verification key\footnote{Depending on the private or public deletion verification setting, we assume that this key is part of $sk$ or $vk$, respectively.} and a deleteable signature, outputs $1$ or $0$.
    \end{itemize}
\end{definition}

\subsection{Simulation Security}
In this section, we define the notion of simulation based deletion security.

\begin{definition}[Simulation Secure Deletion]
    Let $\dss$ be a signature scheme with deletion. We say that $\dss$ satisfies \emph{simulation deletion security} if for any efficient adversary $\adve$, there exists an efficient simulator $\mathsf{Sim}$ such that \\
    \begin{minipage}[t]{.5\linewidth}
    \begin{mdframed}
        {\bf $\underline{\mathsf{REAL}}$}
        \begin{enumerate}[label=\arabic*.]
       
            \item  \textcolor{teal}{$sk, vk \samp \dss.\mathsf{Setup}(1^\lambda)$}
            \item \textcolor{teal}{ $m_1, \dots, m_k, \reg_1 \samp \adve(vk)$}
            \item $sig_i \samp \dss.\mathsf{Sign}(sk, m_i)$ for $i \in [k]$
            \item $\reg_{\mathsf{sig}, i} \samp \dss.\mathsf{Protect}(sk, sig_i)$ for $i \in [k]$
            \item $(\reg_{\mathsf{cert},i})_{i \in [k]}, \reg_2 \samp \adve(\reg, (\reg_{\mathsf{sig},i})_{i \in [k]})$
            \item Execute $\dss.\mathsf{DelVer}(dk, \reg_{\mathsf{cert},i})$ for $i \in [k]$. If any of them fails, output $\perp$. Otherwise, output $\reg_2$.
        \end{enumerate}
    \end{mdframed} 
    \end{minipage}
    $\approx_c$
    \begin{minipage}[t]{.5\linewidth}
    \begin{mdframed}
        {\bf $\underline{\mathsf{SIM}}$}
        \begin{enumerate}[label=\arabic*.]
           
            \item  \textcolor{teal}{$sk, vk \samp \dss.\mathsf{Setup}(1^\lambda)$}
            \item  \textcolor{teal}{$m_1, \dots, m_k, \reg_1 \samp \adve(vk)$}
\item $\reg_2 \samp \mathsf{Sim}^{\mathcal{O}_{sk,\neg\{m_1, \dots, m_k\}}}(vk, (m_i)_{i \in [k]}, \reg_1)$
\item Output $\reg_2$.
        \end{enumerate}
        
    \end{mdframed} 
    \end{minipage}
    where $\mathcal{O}_{sk,\neg\{m_1, \dots, m_k\}}$ denotes the oracle that takes a classical input $m$ and outputs $\dss.\mathsf{Sign}(sk, m)$ if $m \not \in \{m_1, \dots, m_k\}$, and $\perp$ otherwise.
\end{definition}
We can also define the following notion. Note that selective-simulation security is stronger since the simulator has less power.
\begin{definition}[Selective-Simulation Secure Deletion]
      Let $\dss$ be a signature scheme with deletion. We say that $\dss$ satisfies \emph{selective-simulation deletion security} if for any efficient adversary $\adve$, there exists an efficient simulator $\mathsf{Sim}$ such that \\
    \begin{minipage}[t]{.5\linewidth}
    \begin{mdframed}
        {\bf $\underline{\mathsf{REAL}}$}
        \begin{enumerate}[label=\arabic*.]
       
            \item  \textcolor{teal}{$sk, vk \samp \dss.\mathsf{Setup}(1^\lambda)$}
            \item \textcolor{teal}{ $m_1, \dots, m_k, \reg_1 \samp \adve(vk)$}
            \item $sig_i \samp \dss.\mathsf{Sign}(sk, m_i)$ for $i \in [k]$
            \item $\reg_{\mathsf{sig}, i} \samp \dss.\mathsf{Protect}(sk, sig_i)$ for $i \in [k]$
            \item $(\reg_{\mathsf{cert},i})_{i \in [k]}, \reg_2 \samp \adve(\reg, (\reg_{\mathsf{sig},i})_{i \in [k]})$
            \item Execute $\dss.\mathsf{DelVer}(dk, \reg_{\mathsf{cert},i})$ for $i \in [k]$. If any of them fails, output $\perp$. Otherwise, output $\reg_2$.
        \end{enumerate}
    \end{mdframed} 
    \end{minipage}
    $\approx_c$
    \begin{minipage}[t]{.5\linewidth}
    \begin{mdframed}
        {\bf $\underline{\mathsf{SIM}}$}
        \begin{enumerate}[label=\arabic*.]
           
            \item  \textcolor{teal}{$sk, vk \samp \dss.\mathsf{Setup}(1^\lambda)$}
            \item $\regi{sim} \samp \mathsf{Sim}^{\mathcal{O}_{sk}}(vk)$ and let $\mathcal{M}$ be the set of messages queried by $\mathsf{Sim}$.
            \item  \textcolor{teal}{$m_1, \dots, m_k, \reg_1 \samp \adve(vk)$}
            \item If any of the messages $m_i$ for $i \in [k]$ is in $\mathcal{M}$, output $\top$ and terminate.
            \item $\reg_2 \samp \mathsf{Sim}(\regi{sim}, \reg_1, (m_i)_{i \in [k]})$.
            \item Output $\reg_2$.
        \end{enumerate}
        
    \end{mdframed} 
    \end{minipage}
    where $\mathcal{O}_{sk}$ denotes the oracle that takes a classical input $m$ and outputs $\dss.\mathsf{Sign}(sk, m)$.
\end{definition}

We also define a one-time deletion variation of the above definition. In this setting, we restrict to $k = 1$ in the experiments above and the signature scheme is allowed to output a private deletion verification key on a per-signature basis, as part of the output of $\mathsf{Protect}$, and this private key is then sent directly to $\mathsf{DelVer}$ and not to the adversary. In the upcoming sections, we show how to construct scheme that satisfy one-time deletion security, and in \cref{sec:onetomany}, we show how to generically upgrade such schemes to the many-time setting.

\subsection{Game Based Security}
In this section, we define the notion of deletion security against all sound verifiers.
\begin{definition}[Verifier Soundness]
    Let $\dss$ be a signature scheme and let $\mathsf{Ver}$ be a verification algorithm\footnote{Here, we are talking about any algorithm, not just the honest verification procedure of $\dss$.} for $\dss$. Consider the following game between the challenger and an adversary $\adve$.
   
\paragraph{$\underline{\mathsf{FORGE-GAME}_{\dss,\mathsf{Ver}, \adve}(1^\lambda)}$}
\begin{enumerate}
    \item The challenger samples $vk, sk \samp \dss.\mathsf{Setup}(1^\lambda)$.
    \item \textbf{Query Phase:} For multiple rounds, $\adve$ submits a message $m_i$ and the challenger answers by sampling $sig \samp \dss.\mathsf{Sign}(sk, m_i)$ and submitting $sig$ to $\adve$. Let $m_1, \dots, m_k$ be the messages queried by the adversary.
    \item \textbf{Forgery Phase:} The adversary outputs a forged signature $\regi{forged}$ and a message $m^*$. The challenger checks if $m \in \{m_1, \dots, m_k\}$ and outputs $0$ if so. Otherwise, The challenger executes $b \samp \mathsf{Ver}(vk, m^*, \regi{forged})$, and outputs $b$.
\end{enumerate}
We say that $\mathsf{Verify}$ is sound for $\dss$ if for any efficient adversary $\adve$, we have
\begin{equation*}
    \Pr[\mathsf{FORGE-GAME}_{\dss,\mathsf{Ver}, \adve}(1^\lambda) = 1] \leq \negl(\lambda).
\end{equation*}
If the verifier $\mathsf{Ver}$ is sound only against adversaries that output $m^*$ before the query phase, we call it \emph{selective sound}.
\end{definition}

We now define deletion security.
\begin{definition}[Deletion Security]
Let $\dss$ be a signature scheme with deletion, $\mathsf{Ver}$ be a verification algorithm and $\adve$ be an adversary. Consider the following game between the challenger and a \emph{stateful} adversary $\adve$.

\paragraph{$\underline{\mathsf{DEL-GAME}_{\dss,\mathsf{Ver}, \adve}(1^\lambda)}$}
\begin{enumerate}
    \item The challenger samples $vk, sk \samp \dss.\mathsf{Setup}(1^\lambda)$.
    \item \textbf{Query Phase:} For multiple rounds, $\adve$ submits a message $m$ and the challenger answers by sampling $\reg_{\mathsf{sig},i} \samp \dss.\mathsf{Sign}(sk, m)$ and submitting $\regi{sign}$ to $\adve$.
    \item \textbf{Deletion Phase:} The adversary returns a $k$-partite register $(\regi{cert}^i)_{i \in [k]}$ where $k$ is the number of queries it made. The challenger executes $\dss.\mathsf{DelVer}(sk, \regi{cert}^i)$ for all $i \in [k]$. It outputs $0$ and terminates if any of the checks outputs $0$.
    \item \textbf{Forgery Phase:} The adversary outputs a message $m^*$ and a register $\regi{forged}$. The challenger executes $b \samp \mathsf{Ver}(vk, m^*, \regi{forged})$, and outputs $b$.
\end{enumerate}
We say that $\dss$ satisfies \emph{deletion security against sound verifiers} if for any efficient sound verifier $\mathsf{Ver}$ for $\dss$ and any efficient adversary $\adve$, we have
\begin{equation*}
    \Pr[\mathsf{DEL-GAME}_{\dss,\mathsf{Ver}, \adve}(1^\lambda) = 1] \leq \negl(\lambda).
\end{equation*}
\end{definition}

Similar to the simulation security setting, we can also define the notion of one-time deletion security here, where the adversary only makes a single query in the query phase. As in the simulation setting, in this case, we allow the signature scheme to output a deletion verification key along with the signature, but the deletion verification key is not sent to the adversary. 


\section{Construction}
We give a scheme with one-time deletion security. See \cref{sec:onetomany} for generically obtaining multi-signature deletion security.

Let $\css$ be a (post-quantum) classical signature scheme and $\mathsf{AdditiveSh}$ be the additive $n$-out-of-$n$ secret sharing scheme.


\paragraph{$\underline{\mathsf{Setup}(1^\lambda)}$}
\begin{enumerate}
    \item Sample $sk, vk \samp \css.\mathsf{Setup}(1^\lambda)$.
    \item Output $sk, vk$.
\end{enumerate}

\paragraph{$\underline{\mathsf{Sign}(sk, m)}$}
\begin{enumerate}
    \item Sample $x_0^i, x_1^i \samp \zo^{\lambda}$ for $i \in [\ell(\lambda)]$.
    \item Sample $b^i \samp \zo$  for $i \in [\ell(\lambda)]$.
    \item $m^1, \dots, m^{\ell(\lambda)}\samp \mathsf{AdditiveSh}(m, \ell(\lambda))$.
    \item For $i \in [\ell(\lambda)]$,
    \begin{enumerate}[label={\arabic*.}]
    \item $y_0^i = H(x_0^i || m^i)$
    \item  $y_1^i = H(x_1^i  || m^i)$
    \item Sample $sg^i_0 \samp \css.\mathsf{Sign}(sk, y^i_0)$ 
    \item Sample $sg^i_1 \samp \css.\mathsf{Sign}(sk, y^i_1)$.
    \end{enumerate}
    \item $sg \samp \css.\mathsf{Sign}(sk,  (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]})$.
    \item Output $sg, (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, (m_i)_{i \in [\ell]}, (x_0^i, x_1^i, b^i)_{i \in \ell(\lambda)}$.
\end{enumerate}


\paragraph{$\underline{\mathsf{Protect}(sk, sig)}$}
\begin{enumerate}
\item Parse $(sg, (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, (m_i)_{i \in [\ell]}, (x_0^i, x_1^i, b^i)_{i \in \ell(\lambda)}) = sig$
\item Let $\ket{\psi} = \bigotimes_{i \in [\ell(\lambda)]} \frac{\ket{0}\ket{x^i_0} +(-1)^{b^i}\ket{1} \ket{x^i_1}}{\sqrt{2}}$.
    \item Set $\regi{sig} = sg, (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, (m_i)_{i \in [\ell]}, \ket{\psi}$. \textcolor{blue}{// Signature}
    \item Set $dk = (x_0^i, x_1^i, b^i)_{i \in \ell(\lambda)}$. \textcolor{blue}{// Deletion verification key}
    \item Output $\regi{sig}, dk$.
\end{enumerate}

\paragraph{$\underline{\mathsf{DelVer}(dk, \regi{sign})}$}
\begin{enumerate}
    \item Parse $dk = (x_0^i, x_1^i, b^i)_{i \in \ell(\lambda)}$.
    \item Parse $ y, sg, (y_0^i, y^1_i, sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, (m_i)_{i \in [\ell]},  \reg = \regi{sig}$.
    \item Measure $\reg$ projectively onto the state $\bigotimes_{i \in [\ell(\lambda)]} \frac{\ket{0}\ket{x^i_0} +(-1)^{b^i}\ket{1} \ket{x^i_1}}{\sqrt{2}}$. Output $1$ if and only if the measurement succeeds.
\end{enumerate}

\paragraph{$\underline{\mathsf{SigVer}(vk, m, \regi{sig})}$}
\begin{enumerate}
    \item Parse $sg, (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, (m_i)_{i \in [\ell]},  \reg = \regi{sign}$.
    \item Check if $\oplus (m_i) = m$.
    \item Verify $\css.\mathsf{Verify}(vk, (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, sg)$.
    \item Measure $\reg$ in computational basis and parse the result to obtain $(c^i, x^i)_{i \in [\ell(\lambda)]}$ with $|c^i| = 1$ and $|x^i| = \lambda$.
    \item Verify $\css.\mathsf{Verify}(vk, H(x^i || m^i), sg^i_{c^i})$ for $i \in [\ell(\lambda)]$.
    \item Output $1$ if all the verifications passed, otherwise output $0$.
\end{enumerate}



\subsection{Proof of EUF-CMA Security}
\anote{Straightforward}
\subsection{Proof of Deletion Security}\label{sec:delproof}
\anote{We only achieve limited inverse polynomial security for now: We show that for any polynomial $1/p(\lambda)$, we can get a $1/p(\lambda)$ secure scheme by setting the repetition number to $\ell(\lambda) = 5840p^2\log p$}.

Suppose for a contradiction that there exists a selective sound verifier $\mathsf{Ver}$ and an adversary $\adve$ that wins the one-time deletion game with probability $\geq 1/p(\lambda)$. We will show that for some index $i^* \in [\ell(\lambda)]$, we can extract both $x_0^i, x_1^i$ from the signature with non-negligible probability, which is a contradiction by \cref{lem:x0x1}.

At the end of the game, the adversary outputs an $(\ell + 1)$-partite register $\reg_{1}, \reg_{2}, \dots, \reg_{\ell}, \regi{forged}$ where the registers $\reg_{i}$ will be projected (denote the this projection $\Pi_i$) onto $\ket{\psi_i} \vcentcolon= \frac{\ket{0}\ket{x^i_0} +(-1)^{b^i}\ket{1} \ket{x^i_1}}{\sqrt{2}}$ and $\regi{forged}$ will be fed to $\mathsf{Verify}$. Let $\regi{cert} = (\reg_{i})_{i \in {\ell(\lambda)}}$ and $\reg = (\regi{cert}, \regi{forged})$. Let $E_i$ for $i \in [\ell]$ denote the event that the projective measurement on the register $\reg_i$ succeeds, and let $E_{sig}$ denote the event that $\mathsf{Ver}^H(vk, \regi{forged})$ outputs $1$. Observe that the event $E_1 \wedge \dots \wedge E_\ell \wedge E_{sig}$ corresponds to adversary winning, and let $W$ denote this event.

\begin{claim}
    There exists $i^* \in [\ell]$ such that $\Pr[E_{i^*} | E_{{i^*}-1} \wedge \dots \wedge E_1] \geq {1 - \frac{1}{q}}$ where $q = 2920p^2$.
\end{claim}
\begin{proof}
    Suppose otherwise. Then, we have
    \begin{equation*}
        \Pr[E_1 \wedge \dots E_\ell] = \Pr[E_1] \cdot \Pr[E_2 | E_1] \cdots \Pr[E_\ell | E_1 \wedge \dots \wedge E_{\ell - 1}] <  (1-\frac{1}{q})^\ell < \exp(-\frac{\ell}{q}) < 1/p^2.
    \end{equation*}
    However, we also have $\Pr[E_1 \wedge \dots \wedge E_\ell] \geq \Pr[W] \geq 1/p(\lambda)$.
    Thus, we arrive at a contradiction.
\end{proof}

\begin{claim}
    For any $i \in [\ell]$, we have $\Pr[E_{i-1} \wedge \dots \wedge E_1] \geq 1/p(\lambda)$.
\end{claim}
\begin{proof}
    Follows from $\Pr[E_1 \wedge \dots  \wedge E_\ell] \geq \Pr[W] \geq 1/p(\lambda)$.
\end{proof}
\begin{claim}
    For any $i \in [\ell]$, we have $\Pr[E_{sign} | E_{i} \wedge \dots \wedge E_1] \geq 1/p(\lambda)$.
\end{claim}
\begin{proof}
    Follows from $\Pr[E_{sign} | E_{i} \wedge \dots \wedge E_1] \cdot \Pr[E_{i} \wedge \dots \wedge E_1] = \Pr[E_{sign} \wedge E_{i} \wedge \dots \wedge E_1] \geq \Pr[W] \geq 1/p(\lambda)$ and $\Pr[E_{sign} \wedge E_{i} \wedge \dots \wedge E_1] \leq 1$.
\end{proof}

Suppose for now that we know $i^*$. We will show that we can extract $x_0^{i^*}, x_1^{i^*}$ with non-negligible probability, given the signature in the deletion game. Thus, we can obtain a contradiction to \cref{lem:x0x1} by placing the state we get from the challenger in \cref{lem:x0x1} at position $i^*$, and simulating the deletion game and the extraction procedure. During the reduction to \cref{lem:x0x1}, note that we sample on our own an instance the classical scheme $\css$ and sample $x_0^i, x_1^i, b^i$ for $i \in [\ell(\lambda)] \setminus \{i^*\}$. Finally, note that we can actually guess $i^*$ randomly, which will cost us only a polynomial factor loss in the reduction to \cref{lem:x0x1}, which is not an issue.

Now we move onto the extraction procedure. We first simulate the adversary and the deletion game to obtain $\reg = (\regi{cert} = (\reg_{i})_{i \in {\ell(\lambda)}}, \regi{forged})$ as defined above, and then we execute the projections $\Pi_1, \Pi_2, \dots, \Pi_{i^* - 1}$, and if any of them fail, we terminate. Let $\rho$ denote the post-measurement state over $(\regi{forged}, \reg_{i^*})$ conditioned on not terminating. Observe that we can obtain $\rho$ with probability $1/p(\lambda)$ and that it satisfies the following:
\begin{enumerate}
    \item \label{item:firt} Applying $\Pi_{i^*}$ to $\reg_{i^*}$ succeeds with probability $\geq 1 - \frac{1}{q}$,
    \item \label{item:second} Applying $\Pi_{i^*}$ to $\reg_{i^*}$ and conditioning on acceptance, the post-measurement state over $(\regi{forged}, \reg_{i^*})$ (denote it $\tau \otimes \ketbra{\psi_{i^*}}{\psi_{i^*}}$) is such that $\Pr[\mathsf{Ver}^H(vk, \tau) = 1] \geq 1/p(\lambda)$.
\end{enumerate}
Now, since $\Pi_{i^*}$ is a projective measurement, by \cref{lem:gentlemes} and by the claims above, we get \begin{equation}\label{eqn:taupsiclose}
    \trd{\rho}{\tau\otimes \ketbra{\psi_{i^*}}{\psi_{i^*}}} \leq \frac{1}{\sqrt{q}}.
\end{equation}

Now, let $\sigma_c$ for $c \in \zo$ denote the post-measurement state of the register $\regi{forged}$ after measuring the deletion certificate part of the state $\rho$ in the computational basis and conditioning on obtaining the outcome $(c, x_c^{i^*})$. First, observe that we get this outcome (for either value of $c$) with probability $\geq 1/2 - 1/\sqrt{q}$ by \cref{eqn:taupsiclose} and since for $\ket{\psi_{i^*}}$ either outcome occurs with probability exactly $1/2$. Therefore, by \cref{eqn:taupsiclose} and \cref{lem:postmesdistlem}, we get \begin{equation*}
  \trd{\sigma_c}{\tau}   \leq \frac{9}{2\sqrt{q}}.
\end{equation*}
By above we also get
\begin{itemize}
    \item $\trd{\sigma_0}{\sigma_1} \leq \frac{9}{\sqrt{q}}$,
    \item $\Pr[\mathsf{Ver}^H(vk, \sigma_c) = 1] \geq \frac{1}{p(\lambda)} - \frac{9}{2\sqrt{q}} \geq \frac{1}{2\cdot p(\lambda)}$ for $c \in \zo$.
\end{itemize}

We move onto our final argument. Let $r$ be a uniformly random string with the same length as $m$ that we sample. Set $sh' = m \oplus m^{i^*} \oplus r$.
\begin{claim}
    At least one of the following is true.
    \begin{enumerate}
        \item $\qw{\mathsf{Ver}}{H}{(vk, \sigma_{0})}{\{ x^{i^*}_{1}||m^{i^*}, x^{i^*}_{1}||sh'\}}$ is non-negligible,
        \item $\qw{\mathsf{Ver}}{H}{(vk, \sigma_{1})}{\{ x^{i^*}_{0}||m^{i^*}, x^{i^*}_{0}||sh'\}}$ is non-negligible.
        \item $\qw{\mathsf{Ver}}{H'}{(vk, \sigma_{1})}{\{ x^{i^*}_{0}||m^{i^*}, x^{i^*}_{0}||sh'\}}$ is non-negligible where $H'$ denotes the reprogrammed oracle
        \begin{equation*}
        H'(x) = 
            \begin{cases}
                H(x^{i^*}_{1}||m^{i^*}), &\text{ if } x = x^{i^*}_{1}||sh'  \\
                H(x^{i^*}_{1}||sh'), &\text{ if } x = x^{i^*}_{1}||m^{i^*} \\
                H(x), &\text{ otherwise}
            \end{cases}
        \end{equation*}
    \end{enumerate}
\end{claim}
Assume that the claim is true for now and we will prove it later on. Now, we will show that in each case, we can extract $(x^{i^*}_0, x^{i^*}_1)$ with non-negligible probability. In the first case, we proceed as follows. After obtaining $\rho$, we measure the deletion certificate part in the computational basis. With probability $\geq 1/2 - 1/\sqrt{q} \geq 1/3$, we will obtain the outcome $0, x_{0}^{i^*}$ and the state on $\sigma_{0}$ on the signature register. Then, we simulate $\mathsf{Ver}$ on $\sigma_{0}$ and measure a random query of it;  by \cref{lem:qwmeasure}, this gives us $x_{1}^{i^*}$ with non-negligible probability. Thus, we obtain both  $(x^{i^*}_0, x^{i^*}_1)$.
The second case and the third case follow from the same argument as the first case. Only caveat is that in the third case, we simulate $\mathsf{Ver}$ while reprogramming the oracle on the fly at $x^{i^*}_{1}$, that is, whenever passing the queries of $\mathsf{Ver}$ to the actual random oracle, we swap (in superposition) the inputs $x^{i^*}_{1}||m^{i^*}$ and $x^{i^*}_{1}||sh'$. Note that we can actually do this, since we do know $x^{i^*}_{1}$ from our measurement of the deletion certificate, and we sample $r, m^{i^*}$ on our own.

Now we prove the final claim.
\begin{proof}
    Suppose otherwise for a contradiction. Then, we get
   \begin{align}
     \label{eqn:bothnegl}  &\qw{\mathsf{Ver}}{H}{(vk, \sigma_{0})}{\{ x^{i^*}_{1}||m^{i^*}, x^{i^*}_{1}||sh'\}}\leq \negl(\lambda) \\
       &\qw{\mathsf{Ver}}{H}{(vk, \sigma_{1})}{\{ x^{i^*}_{0}||m^{i^*}, x^{i^*}_{0}||sh'\}} \leq \negl(\lambda).\\
           \label{eqn:verhprinegl}   &\qw{\mathsf{Ver}}{H'}{(vk, \sigma_{1})}{\{ x^{i^*}_{0}||m^{i^*}, x^{i^*}_{0}||sh' \}} \leq \negl(\lambda).
   \end{align}
    We first claim $\Pr[\mathsf{Ver}^{H'}(vk, \sigma_0)=1] \geq \frac{1}{4p}$. This follows from \cref{eqn:bothnegl}, $\Pr[\mathsf{Ver}^H(vk, \sigma_0) = 1] \geq 1/(2p(\lambda))$ and \cref{lem:qwtotal}.
    Then, we claim 
    \begin{equation}\label{eqn:sg1vernegl} 
  \Pr[\mathsf{Ver}^{H'}(vk, \sigma_1)=1] \leq \negl(\lambda).      
    \end{equation}
    Observe that once we prove this, we arrive at a contradiction (which means the main claim is true), since this gives us a way of distinguishing $\sigma_0$ versus $\sigma_1$: On input $\sigma$, we simulate $\mathsf{Ver}^{H'}$ on $\sigma$ and output $0$ if it outputs $1$, otherwise we output $0$. By above, this distinguishes $\sigma_0$ versus $\sigma_1$ with advantage $\geq 1/(5\cdot p(\lambda))$, which is a contradiction since $\trd{\sigma_0}{\sigma_1} \leq \frac{9}{\sqrt{q}} \leq 1/(6\cdot p(\lambda))$.

    Now, we prove \cref{eqn:sg1vernegl}. Suppose otherwise. Then, by \cref{eqn:verhprinegl} and \cref{lem:qwtotal}, we get that $\Pr[\mathsf{Ver}^{H''}(vk, \sigma_1) = 1]$ is non-negligible, where we define $H''$
     \begin{equation*}
        H''(x) = 
            \begin{cases}
            H(x^{i^*}_{1}||m^{i^*}), &\text{ if } x = x^{i^*}_{1}||sh'  \\
                H(x^{i^*}_{1}||sh'), &\text{ if } x = x^{i^*}_{1}||m^{i^*} \\
                H(x^{i^*}_{0}||m^{i^*}), &\text{ if } x = x^{i^*}_{0}||sh'  \\
                H(x^{i^*}_{0}||sh'), &\text{ if } x = x^{i^*}_{0}||m^{i^*} \\
                H(x), &\text{ otherwise}
            \end{cases}
        \end{equation*}
 Then, we give the following adversary $\adve'$ that violates the selective soundness of $\mathsf{Ver}$, where we define $sh'' = r_{i^*} \oplus r \oplus m$ and define the reprogramming \begin{equation*}
        H'''(x) = 
            \begin{cases}
            H(x^{i^*}_{1}||r_{i^*}), &\text{ if } x = x^{i^*}_{1}||sh''  \\
                H(x^{i^*}_{1}||sh''), &\text{ if } x = x^{i^*}_{1}||r_{i^*} \\
                H(x^{i^*}_{0}||r_{i^*}), &\text{ if } x = x^{i^*}_{0}||sh''  \\
                H(x^{i^*}_{0}||sh''), &\text{ if } x = x^{i^*}_{0}||r_{i^*} \\
                H(x), &\text{ otherwise}
            \end{cases}
        \end{equation*}
    \paragraph{$\underline{\adve'(vk)}$}
    \begin{enumerate}
    \item Sample $r \samp \zo^{\msglen}$.
    \item Sample $i^* \samp [\ell(\lambda)]$.
    \item Query for a signature on $r$ to get $sig$.
    \item Parse $(sg, (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, (r_i)_{i \in [\ell]}, (x_0^i, x_1^i, b^i)_{i \in \ell(\lambda)}) = sig$.
    \item Run the first stage of $\adve$ to obtain $m, \regi{adv}$.
    \item For $i \in [\ell]$, set $r'_i = m \oplus r_i \oplus r$ if $i = i^*$ and $r'_i = r_i$ otherwise.
    \item Let $\ket{\psi} = \bigotimes_{i \in [\ell(\lambda)]} \frac{\ket{0}\ket{x^i_0} +(-1)^{b^i}\ket{1} \ket{x^i_1}}{\sqrt{2}}$.
    \item Set $\regi{sig} = sg, (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, (r'_i)_{i \in [\ell]}, \ket{\psi}$.
   \item Simulate $\adve^{H'''}(vk, \regi{})$ to obtain $\reg_{1}, \reg_{2}, \dots, \reg_{\ell}, \regi{forged}$.
    \item Execute the projections $\Pi_1, \Pi_2, \dots, \Pi_{i^* - 1}$, and if any of them fail, terminate.
    \item Measure $\reg_{i^*}$ in the computational basis, and terminate if we do not obtain $1, x^{i^*}_1$.
    \item Output $\regi{forged}$.
    \end{enumerate}

    First, observe that we have symmetry between $H$ and $H''$: Both are uniformly random oracles, where $H''$ is obtained from $H$ by swapping the inputs $\{x^{i^*}_{1}||sh' \xleftrightarrow{}  x^{i^*}_{1}||m^{i^*}\}, \{x^{i^*}_{0}||sh' \xleftrightarrow{}  x^{i^*}_{0}||m^{i^*}\}$, and $H$ can be obtained the same way from $H''$. Therefore, we can see that reprogramming the oracle for $\mathsf{Ver}$ is equivalent to keeping the oracle intact for $\mathsf{Ver}$ but reprogramming it for all the other steps (i.e., the adversary $\adve$ and computing the signature for $m$). Further, we have 
    \begin{align*}
        m, i^*, m^1, \dots, &m^\ell, \{m^{i^*}, m\oplus m^{i^*} \oplus r\} \\
        &\equiv \\
        m, i^*, r'_1, \dots, &r'_\ell, \{r'_{i^*}, r_{i^*}\}.
    \end{align*}
    Thus, $\adve'$ playing the forgery game perfectly\footnote{One caveat is that we also need to simulate the first stage of the adversary $\adve$ with $H'''$. However, since the first stage of the adversary $\adve$ does not get the reprogrammed points (which is uniformly random), the difference is exponentially small by \cref{lem:qwtotal}.} simulates (when it does not terminate) $\adve$ getting a signature for $m$ and $\sigma_{1}$ being fed to $\mathsf{Ver}^{H''}$. Thus,
we see that the adversary $\adve'$ wins the soundness game against $\mathsf{Ver}$ with probability \begin{equation*}
       \frac{\Pr[\mathsf{Ver}^{H''}(vk, \sigma_1)=1]}{(1/2 - 1/\sqrt{q})\cdot \ell(\lambda)}
   \end{equation*}
   which would be non-negligible by above. Thus, this is a contradiction to the soundness of $\mathsf{Ver}$. Hence, we have \cref{eqn:sg1vernegl}, which completes the proof.
\end{proof}

\subsection{Proof of Simulation Security}
\anote{Proof sketch. Follows similar to deletion security. Also for now security level depends on repetition parameter.}
We claim that the scheme satisfies $1/p(\lambda)$ selective-simulation security when $\ell(\lambda) = 5840p^2\log p$. 

First, we note that we will only consider adversaries that pass the certificate test (Step 6 of the game $\mathsf{REAL}$) with probability $1/p(\lambda)$, since for other adversaries, the simulator that always outputs $\perp$ directly satisfies $1/p(\lambda)$ simulation security.

For any such adversary $\adve$, as proven in there is an index $i^*$ such that $\Pr[E_{i^*} | E_{{i^*}-1} \wedge \dots \wedge E_1] \geq {1 - \frac{1}{q}}$ where $q = 2920p^2$ as proven in \cref{sec:delproof}. We give the following simulator $\mathsf{Sim}$ for $\adve$\footnote{Note that here we assume we know $i^*$, which makes our reduction non-uniform. We can possibly sample a random $i^*$ instead as in \cref{sec:delproof}} where we define the oracle reprogramming $H'''$:
\begin{equation*}
        H'''(x) = 
            \begin{cases}
            H(x^{i^*}_{1}||r_{i^*}), &\text{ if } x = x^{i^*}_{1}||sh''  \\
                H(x^{i^*}_{1}||sh''), &\text{ if } x = x^{i^*}_{1}||r_{i^*} \\
                H(x^{i^*}_{0}||r_{i^*}), &\text{ if } x = x^{i^*}_{0}||sh''  \\
                H(x^{i^*}_{0}||sh''), &\text{ if } x = x^{i^*}_{0}||r_{i^*} \\
                H(x), &\text{ otherwise}
            \end{cases}
        \end{equation*}
         with $sh'' = r_{i^*} \oplus r \oplus m$.
  \paragraph{$\underline{\mathsf{Sim}(vk)}$}
  \ \\ \textbf{Before obtaining the state of $\adve$:}
    \begin{enumerate}
    \item Sample $r \samp \zo^{\msglen}$.
    %\item Sample $i^* \samp [\ell(\lambda)]$.
    \item Query for a signature on $r$ to get $sig$.
    \item Parse $(sg, (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, (r_i)_{i \in [\ell]}, (x_0^i, x_1^i, b^i)_{i \in \ell(\lambda)}) = sig$.\\ \\
    \textbf{After obtaining the first stage output $\reg, m$ of the adversary:}
    \item For $i \in [\ell]$, set $r'_i = m \oplus r_i \oplus r$ if $i = i^*$ and $r'_i = r_i$ otherwise.
    \item Let $\ket{\psi} = \bigotimes_{i \in [\ell(\lambda)]} \frac{\ket{0}\ket{x^i_0} +(-1)^{b^i}\ket{1} \ket{x^i_1}}{\sqrt{2}}$.
    \item Set $\regi{sig} = sg, (sg^i_0, sg^i_1)_{i \in [\ell(\lambda)]}, (r'_i)_{i \in [\ell]}, \ket{\psi}$.
   \item Simulate $\adve^{H'''}(vk, \regi{})$ to obtain $\reg_{1}, \reg_{2}, \dots, \reg_{\ell}, \regi{forged}$.
    \item Output $\reg_{1}, \reg_{2}, \dots, \reg_{\ell}, \regi{forged}$.
    \end{enumerate}

We claim that for any efficient distinguisher $\mathcal{D}$, we have $|\Pr[\mathcal{D}^{H}(\mathsf{REAL}) = 1] - \Pr[\mathcal{D}^{H}(\mathsf{SIM}) = 1]| \leq 1/p(\lambda)$. Suppose otherwise for a contradiction. Then, we define the following. Let $\sigma_{\mathsf{REAL}, b}$ be the state obtained on the signature register during the modification of the experiment $\mathsf{REAL}$ where we apply the certificate tests $1, \dots, i^* - 1$ and the measure the certificate $i^*$ in the computational basis, and condition on the tests $1, \dots, i^* - 1$ passing and the certificate $i^*$ computational basis measurement giving the outcome $(c, x_c^{i^*})$. Similarly define $\sigma_{\mathsf{SIM}, b}$.
\begin{claim}
    At least one of the following is true.
    \begin{enumerate}
        \item $\qw{\mathcal{D}}{H}{\sigma_{\mathsf{REAL},0}}{\{ x^{i^*}_{1}||m^{i^*}, x^{i^*}_{1}||sh'\}}$ is non-negligible,
        \item $\qw{\mathcal{D}}{H'}{\sigma_{\mathsf{REAL},1}}{\{ x^{i^*}_{0}||m^{i^*}, x^{i^*}_{0}||sh'\}}$ is non-negligible where $H'$ denotes the reprogrammed oracle
        \begin{equation*}
        H'(x) = 
            \begin{cases}
                H(x^{i^*}_{1}||m^{i^*}), &\text{ if } x = x^{i^*}_{1}||sh'  \\
                H(x^{i^*}_{1}||sh'), &\text{ if } x = x^{i^*}_{1}||m^{i^*} \\
                H(x), &\text{ otherwise}
            \end{cases}
        \end{equation*}
    \end{enumerate}
\end{claim}
\begin{proof}
    Suppose otherwise. Then, by \cref{lem:qwtotal}, we get $\mathcal{D}^{H'}(\sigma_{\mathsf{REAL},1}) \approx_{\negl(\lambda)} \mathcal{D}^{H''}(\sigma_{\mathsf{REAL},1})$ where we define $H''$
     \begin{equation*}
        H''(x) = 
            \begin{cases}
            H(x^{i^*}_{1}||m^{i^*}), &\text{ if } x = x^{i^*}_{1}||sh'  \\
                H(x^{i^*}_{1}||sh'), &\text{ if } x = x^{i^*}_{1}||m^{i^*} \\
                H(x^{i^*}_{0}||m^{i^*}), &\text{ if } x = x^{i^*}_{0}||sh'  \\
                H(x^{i^*}_{0}||sh'), &\text{ if } x = x^{i^*}_{0}||m^{i^*} \\
                H(x), &\text{ otherwise}
            \end{cases}
        \end{equation*}

        By the same symmetry argument in \cref{sec:delproof}, we also get $ \mathcal{D}^{H''}(\sigma_{\mathsf{REAL},1}) \equiv \mathcal{D}^{H}(\rho_{\mathsf{SIM}, 1})$.

        We also have $\mathcal{D}^{H'}(\sigma_{\mathsf{REAL},1}) \approx_{9/\sqrt{q}} \mathcal{D}^{H'}(\sigma_{\mathsf{REAL},0})$ since $\sigma_{\mathsf{REAL},0} \approx_{9/\sqrt{q}} \sigma_{\mathsf{REAL},1}$. By $\qw{\mathcal{D}}{H'}{\sigma_{\mathsf{REAL},1}}{\{ x^{i^*}_{0}||m^{i^*}, x^{i^*}_{0}||sh'\}} \leq \negl(\lambda)$, we also get $\mathcal{D}^{H}(\sigma_{\mathsf{REAL},1}) \approx_{9/\sqrt{q}} \mathcal{D}^{H}(\sigma_{\mathsf{REAL},0}) \approx_{\negl(\lambda)} \mathcal{D}^{H'}(\sigma_{\mathsf{REAL},0})$. 
        
        Combining these, we get $\mathcal{D}^{H}(\sigma_{\mathsf{REAL},1}) \approx_{18/\sqrt{q}+\negl(\lambda)} \mathcal{D}^{H}(\sigma_{\mathsf{SIM},1})$. However, this is a contradiction to $|\Pr[\mathcal{D}^{H}(\mathsf{REAL}) = 1] - \Pr[\mathcal{D}^{H}(\mathsf{SIM}) = 1]| > 1/p(\lambda)$.
\end{proof}

Observe that, similar to the argument in \cref{sec:delproof}, in either of the cases above we can extract both $(x_0^{i^*},x_1^{i^*})$ by simulating the modified experiment $\mathsf{REAL}$ and $\mathcal{D}$, obtaining a contradiction to \cref{lem:x0x1}, completing the proof.

\section{One-Time Deletion Security to Multi-Time}\label{sec:onetomany}
Let $\sdss$ be a signature scheme with deletion that satisfies one-time deletion security and $\sesch$ be a secret key encryption scheme with pseudorandom\footnote{We use a scheme with pseudorandom ciphertexts so that the one-time deletion key embedded inside the signature can also be \emph{denied/simulated}.} unforgeable\footnote{That is, we require that an adversary that has obtained multiple ciphertexts $ct_1, \dots, ct_k$ cannot produce $ct' \not\in \{ct_1, \dots, ct_k\}$ such that $\Dec(sk, ct') \neq \perp$, and the ciphertexts are pseudorandom. This can be achieved easily using only pseudorandom functions.} ciphertexts. Then, the following scheme satisfies multi-time deletion security.


\paragraph{$\underline{\mathsf{Setup}(1^\lambda)}$}
\begin{enumerate}
    \item Sample $sk, vk \samp \sdss.\mathsf{Setup}(1^\lambda)$.
    \item Sample $ek \samp \sesch.\mathsf{Setup}(1^\lambda)$.
    \item Output $(sk, ek), vk$.
\end{enumerate}


\paragraph{$\underline{\mathsf{Sign}((sk,ek), m)}$}
\begin{enumerate}
    \item Output $\sdss.\mathsf{Sign}(sk, m)$.
\end{enumerate}

\paragraph{$\underline{\mathsf{Protect}((sk,ek), sig)}$}
\begin{enumerate}
    \item $\rho, dk = \sdss.\mathsf{Protect}(sig)$.
    \item Output $\rho, \sesch.\mathsf{Enc}(ek, dk)$.
\end{enumerate}

\paragraph{$\underline{\mathsf{SigVer}(vk, (\rho, ct))}$}
\begin{enumerate}
    \item Output $\sdss.\mathsf{SigVer}(vk, \rho)$.
\end{enumerate}

\paragraph{$\underline{\mathsf{DelVer}((sk, ek), (\rho, ct))}$}
\begin{enumerate}
\item $dk = \sesch.\mathsf{Dec}(ek, ct)$
\item If $dk = \perp$, output $0$.
    \item Output $\sdss.\mathsf{DelVer}(dk, \rho)$.
\end{enumerate}
 

\section{Current Issues}
\subsection{On Getting a Classical Signature in the Soundness Game}
In the current deletion security definitions, the simulator gets a classical signature on $m$ (or in the game based setting, the verifier soundness is defined with respect to classical signatures, rather than output of $\mathsf{Protect}$). In this section we explain why. Before that, note that this security is still meaningful and non-trivial. Informally, such a security guarantee means that whatever state the adversary has after deletion, it could have been simulated by someone who obtained from the authority a classical signature on $0^\lambda$ or $1^\lambda$, so any sound party should not believe this adversary.

Now we explain the technical reasons. With the current technique for the amplified scheme, we need to be able to apply projections for some of the deletion certificates because we can only conclude that some index is "really good" (i.e. $1-1/q$ good) conditioned on other deletion certificates having been tested and having succeeded, because of the following: If an adversary is winning with probability even some large value such as $1/3$, it is possible that each individual deletion certificate is only $1/3$-good in isolation. Therefore, to get really good certificates, we need conditioning. However, we will also do an extraction on the signature register by simulating the verifier. However, if we do not we get access to the projectors in the soundness game of the verifier, we cannot say anything about this conditioned (i.e. some projections on the other registers having been applied and succeeded) signature state (call it $\rho$), because in the soundness game, we do not get the values $x_0, x_1$ for those other indices we are conditioning on the success of, thus we cannot create $\rho$ in the soundness game. Thus, we cannot conclude any properties of $\rho$ by reducing to the soundnes of the verifier.

A possible solution idea could be to somehow simulate these projections in the verifier's soundness game. For example, maybe we can obtain many signatures on the same message $m$ to simulate both a signature on $m$ and the projectors $\Pi_i$ for various certificate indices, so that we can create $\rho$ (by feeding the signature to adversary and applying the projections to those indices of the output of adversary).
However, if we could simulate obtain projections such an argument (by asking for many signatures on $m$), we would be able to do this in the deletion game too, and in the deletion game having access to projector simulation would break the security since we can project a zero state to obtain the ideal deletion certificate and then measure it learn $x_0, x_1$ (basically, we would be able to create a classical description of a full deleteable signature). Thus, at a minimum, the simulator or the verifier soundness adversary needs to get query access to these projectors. A more straightforward definition is just giving $x_0, x_1$ in the plain in the soundness game.

Another way of looking at it: In the deletion verification with \emph{private} key setting, note that the adversary, after the deletion test, does learn some kind of information on the deletion key, i.e., the test is leaking some information: the fact that the state it submitted passed the projection test.

\subsection{On No-Query Soundness/Simulation}
Note that in the simulation setting, the simulator gets to query for some signatures. In the game based setting, the verifier needs to be sound against adversaries that can query for signatures (note that this is a smaller set of verifiers than \emph{no-query-sound} verifiers).

A question is if we can get no-query simulation. I think we might be able to show that this is impossible in the setting where we have black-box use of the adversaries in the reductions. Note that in the reductions, we are trying to simulate the adversary's behaviour in the deletion game, where it does get some signatures. Can we simulate this without obtianing any signatures at all (but adversary still gets $vk$). Note that for any adversary $\adve$ we are considering, we can also define an adversary $\adve'$ that first tests its input using $vk$, and terminates if it does not validate. $\adve'$ will have the same behaviour as $\adve$ in the deletion game. But we cannot simulate $\adve'$ if we do not obtain any signatures at all.

\section{Technical Lemmata}
\begin{lemma}[Gentle Measurement Lemma \cite{Wildelec}]\label{lem:gentlemes}
    Let $E$ be a POVM element and $\rho$ be a state of appropriate dimension. Suppose the outcome $E$ has a high probability of occuring, that is, $\Tr{E\rho} \geq 1 - \eps$. Then, if we apply a canonical implementation, $\sqrt{E}$, of this measurement, the post-measurement state conditioned on this outcome is close to the original state:
    \begin{equation*}
        \trd{\rho}{\frac{\sqrt{E}\rho\sqrt{E}}{\Tr{E\rho}}} \leq \sqrt{\eps}.
   \end{equation*}
\end{lemma}

\begin{lemma}[Trace Distance Conditioned on Measurement Outcome \cite{CG23}]\label{lem:postmesdistlem}
        Let $M = \{M_i\}_{i \in \mathcal{I}}$ be a general measurement and $\rho, \sigma$ be two states of appropriate dimension such that $\trd{\rho}{\sigma} \leq \eps$.  Let $p_i$ denote probability of outcome $i$ when $M$ is applied to $\rho$, that is $p_i = \Tr{M_i\rho}$. Then,
        \begin{equation*}
            \trd{\rho'}{\sigma'} \leq \frac{3\eps}{2p_i}
        \end{equation*}
        where $\rho', \sigma'$ are post-measurement states conditioned on outcome $i$ when the measurement $M$ is applied to $\rho, \sigma$, respectively. That is, $\rho' = \frac{M_i\rho M_i^\dagger}{\Tr{M_i\rho M_i^\dagger}}$ and $\sigma' = \frac{M_i\sigma M_i^\dagger}{\Tr{M_i\sigma M_i^\dagger}}$.
\end{lemma}

\begin{lemma}\label{lem:unruhperp}\cite{Unruh15}
    Let $\ket{\phi_1} = \ket{\psi} + \ket{\chi_1}$ and $\ket{\phi_2} = \ket{\psi} + \ket{\chi_2}$ for (unnormalized) quantum states such that $\ket{\chi_1} \perp \ket{\psi}$ and $\ket{\chi_2} \perp \ket{\psi}$. Then, $\trd{\ket{\phi_1}}{\ket{\phi_2}} \leq 2\norm{\ket{\chi_1}}$.
\end{lemma}

\begin{lemma}\label{lem:x0x1}
    For any adversary $\adve$ that makes polynomially many queries to the random oracle, we have
    \begin{equation*}
        \Pr[x'_0 = x_0 \wedge x'_1 = x_1 : \begin{array}{c}
            H \samp (\zo^{n(\lambda)} \to \zo^{m(\lambda}) \\
             b \samp \zo \\
            x_0, x_1 \samp \zo^{\lambda} \\
            x'_0, x'_1 \samp \adve^H\left(\frac{\ket{0}\ket{x_0} + (-1)^{b}\ket{1}\ket{x_1}}{\sqrt{2}}, H(x_0), H(x_1)\right)
        \end{array}] \leq \negl(\lambda).
    \end{equation*} 
\end{lemma}
\begin{proof}
    \anote{Write down the density matrices}.
\end{proof}
\subsection{Quantum Random Oracle (QROM) Results}
\anote{We can kind of get QROM with any output length by $H'(x) = H(x || BINARY(0)) || H(x ||  BINARY(1)) || \dots H(x ||  BINARY(n))$, but there are problems with it}

\begin{definition}[Query Weight]
    Let $\mathcal{B}$ be an oracle algorithm, $H: \zo^{n(\lambda)} \to \zo^{m(\lambda)}$ be an (possibly random) oracle, $S$ be a (possibly random) set of inputs and $\rho$ be a (possibly correlated with $H, S$) state. We write $\qw{\mathcal{B}}{H}{\rho}{S}$ to denote the total query weight of $\mathcal{B}$ on the set $S$ when it is run on the input $\rho$, write $\qwt{\mathcal{B}}{H}{\rho}{S}{t}$ to denote the query weight at $t$-th query.

    More precisely, suppose $\rho = \sum_{H,S,j} p_{H,S,j} \ketbra{\psi^{H,S,j}_0}{\psi^{H,S,j}_0}$ and suppose $\mathcal{B}$ makes $T$ queries to the oracle $H$, and let $\ket{\psi^{H,S,j}_t} = \sum_{w,x,b} \alpha^{t,H,S,j}_{w,x,b} \ket{w,x,b} = (UU^H)^t \ket{\psi^{H,S,j}_0}$ for $t \in [T]$ be the $t$-th query of the algorithm (written as a state over the workspace, query input and query output registers respectively) on input $\rho$ for a fixing $H,S,j$ of the randomness. Then,
    \begin{align*}
        &\qwt{\mathcal{B}}{H}{\rho}{S}{t} = \E_{H,S,j}\left[\sum_{x \in S} \sum_{w,b}|\alpha^{t,H,S,j}_{w,x,b}|^2 \right] \\
        &\qw{\mathcal{B}}{H}{\rho}{S} = \sum_t \qwt{\mathcal{B}}{H}{\rho}{S}{t}.
    \end{align*}
\end{definition}
We now present the following results. They can be seen as slight generalizations and splitting into two of the one-way-to-hiding lemma \cite{Unruh15}, and they follow from a similar argument.
\begin{lemma}[Query Weight - Distinguishing Advantage Lemma]\label{lem:qwtotal}
    Let $H: \zo^{n(\lambda)} \to \zo^{m(\lambda)}$ denote an (possibly random) oracle and let $\mathcal{B}_1, \mathcal{B}_2$ be two (quantum) oracle algorithms. Then,
    \begin{align*}
       \mathsf{Adv} =\bigg\| &\left((\mathcal{B}^H_2(\rho), H, H', S, Y): 
            \rho, S, Y \samp \mathcal{B}^H_1(1^\lambda)
           \right) - \\  &\left((\mathcal{B}^{H'}_2(\rho), H, H', S, Y) :
            \rho, S, Y \samp \mathcal{B}^H_1(1^\lambda)
           \right)\bigg\|_{Tr} \leq 2\sqrt{T}\cdot\sqrt{\qw{\mathcal{B}_2}{H}{\mathcal{B}_1(1^\lambda, S)}{S}}.
    \end{align*}
    where we write $S = (x_1, \dots, x_{s(\lambda)}), Y =  (y_1, \dots, y_{s(\lambda)})$ and \begin{equation*}
        H'(x) = \begin{cases}
            H(x), \text{ if } x \not\in S,\\
            y_i, \text{ if } x=x_i \text{ for } i \in [s(\lambda)]
        \end{cases}
    \end{equation*}
\end{lemma}
\begin{proof}
To bound this trace distance between these two states $\sigma_1, \sigma_2$, we will show that the trace distance between the states in both cases can only grow by the query weight on $S$ during each query.

To bound $\trd{\sigma_1}{\sigma_2}$, we will first bound the distance by the total query weight for each fixing of the randomness, then a Jensen's inequality argument will yield the final result. Also note that we will ignore the $H, H', S, Y$ part since it is the same in both states.
Let $\sum_{H, S, Y, j}p_{H,S,Y,j}{\ketbra{\phi_{H,S,Y,j}}{\phi_{H,S,Y,j}}}\otimes\ketbra{S}{S}\otimes\ketbra{Y}{Y}$ be a decomposition of the output of $\mathcal{B}^H_1(1^\lambda)$. Consider any fixing of $S, H, Y, j$. Let $U^H$ denote the oracle unitary for $H$ (i.e. $\ket{w, x, b} \to \ket{w,x,b \oplus H(x)}$) and let $U$ be the evolution unitary of $\mathcal{B}_2$. Let $\ket{\psi_t}, \ket{\psi'_t}$ be the state after the $t$-th query when $\mathcal{B}_2$ is run on $H, H'$ respectively. That is, $\ket{\psi_t} = (UU^H)^t,\ket{\psi'_t} = (UU^{H'})^t$, and $\ket{\psi_0} = \ket{\psi'_0} = U(\ketbra{\phi_{H,S,Y,j}}\otimes\ket{0}^{w(\lambda)})$.

Define $D_t = \trd{\ket{\psi_t}}{\ket{\psi'_t}}$. We have
\begin{align*}
    D_t &= \trd{\ket{\psi_t}}{\ket{\psi'_t}} \\
    &= \trd{UU^H\ket{\psi_{t-1}}}{UU^{H'}\ket{\psi'_{t-1}}} \\
    &\leq \trd{UU^H\ket{\psi_{t-1}}}{UU^{H'}\ket{\psi_{t-1}}} + \trd{UU^{H'}\ket{\psi_{t-1}}}{UU^{H'}\ket{\psi'_{t-1}}}
    \\ &= \trd{U^H\ket{\psi_{t-1}}}{U^{H'}\ket{\psi_{t-1}}} + D_{t-1}.
\end{align*}

Now, for any $x$, define  $\Pi_{x}$ to be the projector (defined over all registers) $\ketbra{x}{x}\otimes I$ onto the basis element $\ket{x}$  of the query input register and $U_y$ to be the unitary mapping $\ket{w,x,b}\to \ket{w,x,b\oplus y}$. Also define $H^{(i)}$ for $i \in \{0,\dots, s\}$ to be \begin{equation*}
        H^{(i)}(x) = \begin{cases}
            H(x), \text{ if } x \not\in \{x_1, \dots, x_i\},\\
            H'(x) , \text{ if } x \in \{x_1, \dots, x_i\}
        \end{cases}
    \end{equation*}
    Observe that we have $H^{(0)}=H$ and $H^{(s)}=H'$. Then, we have
    \begin{align*}
        &\trd{U^H\ket{\psi_{t-1}}}{U^{H'}\ket{\psi_{t-1}}} \leq \\ &\trd{U^{H^{(0)}}\ket{\psi_{t-1}}}{U^{H^{(1)}}\ket{\psi_{t-1}}} + \trd{U^{H^{(1)}}\ket{\psi_{t-1}}}{U^{H^{(2)}}\ket{\psi_{t-1}}} + \dots + \trd{U^{H^{(s-1)}}\ket{\psi_{t-1}}}{U^{H^{(s)}}\ket{\psi_{t-1}}}
    \end{align*}

    We claim $\trd{U^{H^{(i)}}\ket{\psi_{t-1}}}{U^{H^{(i+1)}}\ket{\psi_{t-1}}} \leq 2\norm{\Pi_{x_i}\ket{\psi_{t-1}}}$. First, observe that we can write $U^{H^{(i+1)}} = U^{H^{(i)}}(I - \Pi_{x_{i+1}}) + U_{y_{i+1}}\Pi_{x_{i+1}}$. Thus, we have 
    \begin{align*}
        &\trd{U^{H^{(i)}}\ket{\psi_{t-1}}}{U^{H^{(i+1)}}\ket{\psi_{t-1}}}  \\&= 
        \trd{\left(U^{H^{(i)}}(I - \Pi_{x_{i+1}}) \ket{\psi_{t-1}} + U^{H^{(i)}} \Pi_{x_{i+1}}\ket{\psi_{t-1}}\right)} {\left(U^{H^{(i)}}(I - \Pi_{x_{i+1}})\ket{\psi_{t-1}} +  U_{y_{i+1}}\Pi_{x_{i+1}}\ket{\psi_{t-1}}\right)}\\ &\leq
         2\norm{ U_{y_{i+1}}\Pi_{x_{i+1}}\ket{\psi_{t-1}}} =  2\norm{\Pi_{x_{i+1}}\ket{\psi_{t-1}}}
    \end{align*}
    by \cref{lem:unruhperp} since $ U_{y_{i+1}}\Pi_{x_{i+1}}\ket{\psi_{t-1}} \perp U^{H^{(i)}}(I - \Pi_{x_{i+1}})\ket{\psi_{t-1}} $ and $U^{H^{(i)}}(I - \Pi_{x_{i+1}})\ket{\psi_{t-1}}  \perp  U^{H^{(i)}} \Pi_{x_{i+1}}\ket{\psi_{t-1}}$. Thus, we get $\trd{U^{H^{(i)}}\ket{\psi_{t-1}}}{U^{H^{(i+1)}}\ket{\psi_{t-1}}} \leq 2 {\norm{\sum_{i \in [s]}\Pi_{x_{i}}\ket{\psi_{t-1}}}}$ by observing that the elements $\{\Pi_{x_i}\ket{\psi_{t-1}}\}_{i \in [s]}$ are mutually orthogonal.

    Also observe that $\sum_{i \in [s]}\norm{\Pi_{x_i}\ket{\psi_{t-1}}}^2$ is the total query weight on $S$ during the $t$-th query. Thus, we have 
    \begin{align*}
        \mathsf{Adv} &\leq \sum_{H, S, Y, j}p_{H,S,Y,j} D_T(H,S,Y,j) \\
        &\leq 2T \cdot \sum_{H, S, Y, j; t \in [T]}\frac{p_{H,S,Y,j}}{T} {\norm{\sum_{i \in [s]}\Pi_{x_{i}}\ket{\psi^{H,S,Y,j}_{t-1}}}} \\
        &\leq 2T \cdot \sqrt{ \sum_{H, S, Y, j; t \in [T]}\frac{p_{H,S,Y,j}}{T} {\norm{\sum_{i \in [s]}\Pi_{x_{i}}\ket{\psi^{H,S,Y,j}_{t-1}}}}^2} \\
     &= 2\sqrt{T}\cdot\sqrt{\qw{\mathcal{B}_2}{H}{\mathcal{B}_1(1^\lambda)}{S}}.
    \end{align*}
    First line is by joint convexity of trace distance, third line is by Jensen's inequality.
\end{proof}

\begin{lemma}[Query Weight - Extraction Lemma]\label{lem:qwmeasure}
    Let $H: \zo^{n(\lambda)} \to \zo^{m(\lambda)}$ denote an oracle, $\rho$ denote a state and $S$ denote a set of inputs, all possibly correlated.
    
    Suppose $\mathcal{B}$ makes at most $T(\lambda)$ queries to $H$ on input $\rho$. Then, there exists $\mathcal{E}$ such that on input $\rho$, it outputs a value $(x, y)$ satisfying $H(x) = y$ and $x \in S$ with probability at least \begin{equation*}
        \frac{\qw{\mathcal{B}}{H}{\rho}{S}}{T^2}.
    \end{equation*}
\end{lemma}
\begin{proof}
   First, since we have $\sum_{t \in [T]}{\qwt{\mathcal{B}}{H}{\rho}{S}{t}} = \qw{\mathcal{B}}{H}{\rho}{S}$, there must be $t^*$ such that $\qwt{\mathcal{B}}{H}{\rho}{S}{t^*} \geq \frac{\qw{\mathcal{B}}{H}{\rho}{S}}{T}$. Also note that measuring the query $t^*$ gives us $x \in S$ with probability $\qwt{\mathcal{B}}{H}{\rho}{S}{t^*}$. Thus, simulating $\mathcal{B}$, stopping it after a randomly chosen index and measuring its query gives us the desired result.
\end{proof}





==> Notes/updated_lemmas.tex <==
\section{Updated Lemmas}

\begin{lemma}[Double Extraction problem]
    For all QPT oracle algorithms $A^{(\cdot)}$ with auxiliary input $\rho$, the probability of winning the following game is negligible:
    \begin{enumerate}
        \item Sample $x_0, x_1\gets \{0,1\}^\lambda$ and $b\gets \{0,1\}$. Sample a random oracle $H$ and send the following to $A$:
        \[
            H(x_0),\ H(x_1),\ \ket{x_0} + (-1)^b\ket{x_1}
        \]
        \item $A^H(\rho,  H(x_0),\ H(x_1),\ \ket{x_0} + (-1)^b\ket{x_1})$ wins if it outputs $x_0$ and $x_1$.
    \end{enumerate}
\end{lemma}

\paragraph{2 Stage Verifier Lemmas} A two-stage verifier $V_{P}(\rho_V)$ consists of two binary PVMs $P$ and $V$ and an internal register $\cV$ which is intialized to an auxiliary input state $\rho_V$. On input a state $\ket{w}$ it applies $P$ to $\ket{w}$ and its internal register $\cV$, then applies $V$ to $\ket{w}$ and $\cV$. It outputs accept if and only if both measurements output accept. If the verifier requires oracle access to $H$, then both projections receive access to the same oracle $H$.

\begin{lemma}\label{lem:soundVamplification}
    Let $V(\rho_V)$ be a sound verifier and let $A$ be an adversary such that $(A, V(\rho_V))$ win the certified deniability game with noticeable probability. If there exists an efficient projector $\Pi_{\rho_V}$ onto $\rho_V$, then there exists a sound two-stage verifier $\widetilde{V}_{\widetilde{V}}(\rho_V)$ such that:
    \begin{enumerate}
        \item $(A, \widetilde{V}_{\widetilde{V}}(\rho_V))$ win the certified deniability game with noticeable probability.
        \item Conditioned on $\widetilde{V}$ outputting accept on a register $\cR$, a second application of it to $\cR$ outputs accept with $1-\negl$ probability.
    \end{enumerate}
    \justin{The requirement that  $\Pi_{\rho_V}$ is efficient could be an issue for the general case.}
\end{lemma}
\begin{proof}[Proof Sketch]
    \justin{TODO. Intuition is that $\rho_w\otimes \rho_V$ must lie within Jordan subspaces where the eigenvectors of $V$ and $\Pi_{\rho_V}$ are far from each other. This means that Marriot-Watrous amplification on $\rho_w\otimes \rho_V$ using $V$ and $\Pi_{\rho_V}$ should reject with overwhelming probability. Could be more complicated for mixed states vs pure states.}
\end{proof}

\begin{lemma}
    Let $V^H_{P^H}(\rho_V)$ be a sound verifier with oracle access to $H$ and consider an adversary $A^H$ which receives a signature on $m$, then outputs a state $\rho^{\cert, \sig}$. If the following conditions hold, then there exists a QPT oracle algorithm that wins the double extraction problem with noticeable probability.
    \begin{enumerate}
        \item The probability of $P^H$ accepting register $\sig$ of $\rho^{\cert, \sig}$ is noticeable. Let $\restr{\rho}{P}$ denote the renormalized state after $P^H$ accepts $\rho^{\cert, \sig}$.
        \item The probability of the certificate check accepting register $\cert$ of $\restr{\rho}{P}$ is noticeable. Let $\restr{\rho}{P,\cert}$ denote the renormalized state after $\restr{\rho}{P}$ passes this check.
        \item The probability of $V^H$ accepting register $\sig$ of $\restr{\rho}{P,\cert}$ is at least $\omega\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right)$.
    \end{enumerate}

    \justin{This lemma is very unlikely to be true. See the proof sketch for details.}

    \justin{A possible fix is to require that soundness holds even if $P$ and $V$ use different oracles. However, this would require an updated version of \Cref{lem:soundVamplification} which I doubt is true in general.}
\end{lemma}

\paragraph{Remark: Non-Oracle Version.} In the non-oracle version, $V$, $P$, and $A$ do not use oracle access to $H$. However, we cannot hope to actually prove the non-oracle version because we use the oracle in a fundamental way to do the extraction.

% \paragraph{Remark: Combining the Two Lemmas.} If $\widetilde{V}^H$ accepts with $1-\negl$ probability, then conditioned on any event that occurs with noticeable probability, it still accepts with $1-\negl$ probability. Thus, after conditioning on the certificate check passing, $\widetilde{V}^H$ still accepts with overwhelming probability, which is certainly $\omega\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right)$. Furthermore, $P^H$ and the certificate check are applied to different registers, so they commute

\begin{proof}[Proof Sketch]
    There are several steps to the proof. First, condition on $P^H$ accepting the signature register, so that the state of the system is $\restr{\rho}{P}$. Then:
    \begin{enumerate}
        \item Show that there is an index $i^*$ where the certificate is very good conditioned on the others accepting - it should accept with probability $1 - O\left(\frac{\log(\lambda)}{\lambda}\right)$. This is a straightforward probability calculation.
        
        \item Use step 1 to show that after extracting some $x_{i^*}^b$ from the \emph{certificate register}, the leftover signature register is still $O\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right)$-far in trace distance from its original state. This implies:
        \begin{enumerate}
            \item The state of the signature register $\sigma_0$ after extracting $x_{i^*}^0$ from the certificate register is $O\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right)$-far from its state $\sigma_1$ after extracting $x_{i^*}^1$. This gives a bound on the probability of distinguishing $\sigma_0$ and $\sigma_1$.
            \item The probability of $V^H_{P^H}(\rho_V)$ accepting $\sigma_0$ is $\omega\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right) - O\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right) = \omega\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right)$.
        \end{enumerate}
        This step is also straightforward using gentle-measurement-style lemmas.

        \item Extract $x_{i^*}^{1-b}$ from the signature register.\footnote{In the actual reduction, we take a poly loss by guessing the index $i^*$.} This is a multi-step process that reasons about the behavior of $V^{(\cdot)}$ on three different oracles:
        \begin{itemize}
            \item The original oracle $H$. Step 2 implies that $V^H$ accepts with $\omega\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right)$ probability if $b=0$, i.e. when $x_{i^*}^0$ is extracted from the certificate register.
            \item An oracle $H'_{x_{i^*}^0, x_{i^*}^1}$, which is reprogrammed at both $x_{i^*}^0$ and $x_{i^*}^1$ so that the signature that the adversary received is invalid. {\color{red} In the original proof, we used $V$'s soundness to show that it will reject with overwhelming probability, since the adversary never received a signature that is valid with respect to $H'_{x_{i^*}^0, x_{i^*}^1}$. However, here we \emph{already applied} $P^H$, and soundness only holds if $P$ and $V$ use the same oracle.}
            \item An intermediate oracle $H'_{x_{i^*}^1}$ which matches $H'_{x_{i^*}^0, x_{i^*}^1}$ at $x_{i^*}^1$ and matches $H$ at all other points.
        \end{itemize}
        Since $V^{(\cdot)}$ behaves very differently on $H$ and $H'_{x_{i^*}^0, x_{i^*}^1}$, it must either be able to distinguish (a) between $H$ and the intermediate oracle $H'_{x_{i^*}^1}$ or (b) between the intermediate oracle $H'_{x_{i^*}^1}$ and $H'_{x_{i^*}^0, x_{i^*}^1}$, both with advantage $\omega\left( \sqrt{\frac{\log(\lambda)}{\lambda} }\right)$. Here is the case analysis:
        \begin{enumerate}
            \item Say $V^{(\cdot)}$ can distinguish between $H$ and the intermediate oracle $H'_{x_{i^*}^1}$ after $x_{i^*}^0$ is extracted from the certificate register. Then we can immediately extract $x_{i^*}^1$ from the signature register with noticeable probability, which wins us the double extraction game.
            \item Say $V^{(\cdot)}$ can distinguish between the intermediate oracle $H'_{x_{i^*}^1}$ and $H'_{x_{i^*}^0, x_{i^*}^1}$ after $x_{i^*}^0$ is extracted from the certificate register, i.e. using $\sigma_0$. 
            Then we show that $V^{(\cdot)}$ can \emph{also} distinguish between these oracle using $\sigma_1$ with noticeable probability, or else we can distinguish between $\sigma_0$ and $\sigma_1$ with advantage $\omega\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right)$, which is better than is allowed by the $O\left(\sqrt{\frac{\log(\lambda)}{\lambda}}\right)$ distance between them. 
            
            Since $V$ can distinguish between these oracles using $\sigma_1$ with noticeable probability, whenever we extract $x_{i^*}^1$ from the certificate register, we can extract $x_{i^*}^0$ from the signature register with noticeable probability, which wins the double extraction game.
        \end{enumerate}
        
    \end{enumerate}
\end{proof}
